SpiderBoost and Momentum: Faster Stochastic Variance Reduction Algorithms

SARAH and SPIDER are two recently developed stochastic variance-reduced algorithms, and SPIDER has been shown to achieve a near-optimal first-order oracle complexity in smooth nonconvex optimization. However, SPIDER uses an accuracy-dependent stepsize that slows down the convergence in practice, and cannot handle objective functions that involve nonsmooth regularizers. In this paper, we propose SpiderBoost as an improved scheme, which allows to use a much larger constant-level stepsize while maintaining the same near-optimal oracle complexity, and can be extended with proximal mapping to handle composite optimization (which is nonsmooth and nonconvex) with provable convergence guarantee. In particular, we show that proximal SpiderBoost achieves an oracle complexity of $\mathcal{O}(\min\{n^{1/2}\epsilon^{-2},\epsilon^{-3}\})$ in composite nonconvex optimization, improving the state-of-the-art result by a factor of $\mathcal{O}(\min\{n^{1/6},\epsilon^{-1/3}\})$. We further develop a novel momentum scheme to accelerate SpiderBoost for composite optimization, which achieves the near-optimal oracle complexity in theory and substantial improvement in experiments.

==> Experiments.tex <==
\section{Experiments}
To illustrate the idea of large step size, we present following demo experiments. We use SPIDER and SPIDER$^\textbf{+}$ to solve a logistic regression problem with a non convex regularizer. Both algorithms use the same parameter setting expect the step size. To achieve a first order stationary point with $\|\nabla f(x)\| \leqslant 0.1$, we set   $\eta = 0.1$ in SPIDER and $\eta = 0.8$ in SPIDER$^\textbf{+}$   according to the suggestion in their convergence theorem. We point out two observations. (i) the  gradient norm of points generated by  SPIDER oscillating around  $0.1$, which also justifies that a more large step size may cause large oscillating in SPIDER, and hence $\eta = 0.1$  is reasonable large for SPIDER. (ii) SPIDER$^\textbf{+}$  is much faster than SPIDER due to the allowance of a  much large step size. 
\begin{figure*}[ht]  
	\vspace{-0.3cm}
	\centering 
	\subfigure[Gradient]{\includegraphics[width=0.45\linewidth]{figs/grad.pdf}}   
	\subfigure[Loss]{\includegraphics[width=0.45\linewidth]{figs/loss.pdf}}  
	\caption{Nonconvex logistic regression. Left: gradient norm v.s. SFO. Bottom: function value gap v.s. SFO. }   \label{Experment_1}
\end{figure*}

==> convergence_proximal_spiderM_-_Copy.tex <==

{\Large{\bf Supplementary Materials}}
\section{Auxiliary Lemmas for Analysis of \Cref{alg: ProxSPIDERM}}
In this section, we collect some auxiliary results that facilitate the analysis of Prox-SpiderBoost-M. 
Throughout, for any $k\in \mathbb{N}$, denote $\tau(k) \in \mathbb{N}$ the unique integer such that $(\tau(k)-1)q \le k \le \tau(k) q - 1$. We also define $\Gamma_0 = 0, \Gamma_1 = 1$ and $\Gamma_k = (1-\alpha_k)\Gamma_{k-1}$ for $k=2,3,...$. Since we set $\alpha_k = \frac{2}{\ceil[]{k/q}+1}$, it is easy to check that $\Gamma_k = \frac{2}{\ceil[]{k/q}(\ceil[]{k/q}+1)}$.

We first present an auxiliary lemma from \cite{Fang2018}.
\begin{lemma}{\cite{Fang2018}}\label{lemma: Zhang}
	Under \Cref{assum: f}, the estimation  $v_k$ of gradient constructed by SPIDER satisfies that for all $(\tau(k)-1)q +1 \le k \le \tau(k)q-1$,
	\begin{align*}
	\mathbb{E} \|v_k - \nabla f(z_k)\|^2 &\le \frac{L^2}{|\xi_k|} \mathbb{E}\|z_k - z_{k-1}\|^2 +\mathbb{E}\|v_{k-1} - \nabla f(z_{k-1})\|^2.
	\end{align*}
\end{lemma}


Telescoping \Cref{lemma: Zhang} and noting that $v_k = \nabla f(z_k)$ for all $k$ such that $\textrm{mod}(k,q) =0$, we obtain the following bound.
\begin{lemma}\label{aux: 1}
	Under \Cref{assum: f}, the estimation  $v_k$ of gradient constructed by SPIDER satisfies that for all $k\in \mathbb{N}$,
	\begin{align}
	\mathbb{E} \|v_k - \nabla f(z_k)\|^2 \le \sum_{i=(\tau(k)-1)q}^{k-1}\frac{L^2}{|\xi_i|} \mathbb{E}\|z_{i+1} - z_{i}\|^2. \label{eq: variance bound}
	\end{align}
\end{lemma}

Next, recall the following definition of the gradient mapping for some $\eta>0$ and $x, u \in \mathbb{R}^d$:
\begin{align*}
	G_\eta(x,u) := \frac{1}{\eta} \big(x-\mathrm{prox}_{\eta g}(x-\eta u) \big).
\end{align*}
Based on this definition, we can rewrite the updates of \Cref{alg: ProxSPIDERM} as follows:
\begin{align}
	z_{k} &= (1-\alpha_{k+1})y_{k} + \alpha_{k+1} x_{k}, \nonumber\\
	x_{k+1} &=  x_k - \lambda_{k} G_{\lambda_k}(x_k, v_k), \nonumber\\
    y_{k+1} &= z_{k} - \beta_{k} G_{\lambda_k}(x_k, v_k). \nonumber
\end{align}
Next, we prove the following auxiliary lemma. 
\begin{lemma}\label{aux: 3}
	Let the sequences $\{x_k\}_k, \{y_k\}_k, \{z_k\}_k$ be generated by \Cref{alg: ProxSPIDERM}. Then, the following inequalities hold
	\begin{align}
	y_k - x_k &= \Gamma_k\sum_{t=1}^k \frac{\lambda_{t-1} - \beta_{t-1}}{\Gamma_t} G_{\lambda_{t-1}}(x_{t-1}, v_{t-1}),\\
	\|y_k - x_k\|^2 &\le \Gamma_k\sum_{t=1}^k \frac{\lambda_{t-1} - \beta_{t-1}}{\alpha_t\Gamma_t} \|G_{\lambda_{t-1}}(x_{t-1}, v_{t-1})\|^2,\\
	\|z_{k+1}-z_k\|^2 &\le 2\beta_{k}^2\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + 2\alpha_{k+2}^2 \Gamma_{k+1}\sum_{t=1}^{k+1} \frac{(\lambda_{t-1} - \beta_{t-1})^2}{\alpha_t\Gamma_t} \|G_{\lambda_{t-1}}(x_{t-1}, v_{t-1})\|^2.
	\end{align}
\end{lemma}
\begin{proof}
	We prove the first equality. By the update rule of the momentum scheme, we obtain that
	\begin{align}
	y_k - x_k &= z_{k-1} - \beta_{k-1} G_{\lambda_{k-1}}(x_{k-1}, v_{k-1}) - (x_{k-1} - \lambda_{k-1} G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})) \nonumber\\
	&= (1-\alpha_k) (y_{k-1} - x_{k-1}) + (\lambda_{k-1} - \beta_{k-1}) G_{\lambda_{k-1}}(x_{k-1}, v_{k-1}). 
	\end{align}
	Dividing both sides by $\Gamma_k$ and noting that $\frac{1-\alpha_k}{\Gamma_k} = \frac{1}{\Gamma_{k-1}}$, we further obtain that
	\begin{align}
	\frac{y_k - x_k}{\Gamma_k} &= \frac{y_{k-1} - x_{k-1}}{\Gamma_{k-1}} + \frac{\lambda_{k-1} - \beta_{k-1}}{\Gamma_k} G_{\lambda_{k-1}}(x_{k-1}, v_{k-1}). 
	\end{align}
	Telescoping the above equality over $k$ yields the first desired equality. 
	
	Next, we prove the second inequality. Based on the first equality, we obtain that
	\begin{align}
	\|y_k - x_k \|^2 &= \|\Gamma_{k} \sum_{t=1}^{k} \frac{\lambda_{t-1} - \beta_{t-1}}{\Gamma_t} G_{\lambda_{t-1}}(x_{t-1}, v_{t-1})\|^2 \nonumber \\
	&= \|\Gamma_{k} \sum_{t=1}^{k} \frac{\alpha_t}{\Gamma_t} \frac{\lambda_{t-1} - \beta_{t-1}}{\alpha_t} G_{\lambda_{t-1}}(x_{t-1}, v_{t-1})\|^2 \nonumber \\
	&\overset{(i)}{\le} \Gamma_{k} \sum_{t=1}^{k} \frac{\alpha_t}{\Gamma_t} \frac{(\lambda_{t-1} - \beta_{t-1})^2}{\alpha_t^2}  \|G_{\lambda_{t-1}}(x_{t-1}, v_{t-1})\|^2 \nonumber \\
	&= \Gamma_{k} \sum_{t=1}^{k} \frac{(\lambda_{t-1} - \beta_{t-1})^2}{\Gamma_t\alpha_t}  \|G_{\lambda_{t-1}}(x_{t-1}, v_{t-1})\|^2,
	\end{align}
	where (i) uses the facts that $\{\Gamma_k\}_k$ is a decreasing sequence, $\sum_{t=1}^{k} \frac{\alpha_t}{\Gamma_t} = \frac{1}{\Gamma_k}$ and Jensen's inequality.
	
	Finally, we prove the third inequality. By the update rule of the momentum scheme, we obtain that $z_{k+1} - z_{k} = y_{k+1} - z_k + \alpha_{k+2} (x_{k+1} - y_{k+1})$. Then, we further obtain that
	\begin{align}
	\|z_{k+1} - z_{k}\| &\le \|y_{k+1} - z_k\| + \alpha_{k+2} \|x_{k+1} - y_{k+1}\| \nonumber \\
	&\le \beta_{k} \|G_{\lambda_k}(x_k, v_k)\| + \alpha_{k+2} \sqrt{\|x_{k+1} - y_{k+1}\|^2} \nonumber \\
	&\le \beta_{k} \|G_{\lambda_k}(x_k, v_k)\| + \alpha_{k+2} \sqrt{\Gamma_{k+1} \sum_{t=1}^{k+1} \frac{(\lambda_{t-1} - \beta_{t-1})^2}{\Gamma_t\alpha_t}  \|G_{\lambda_{t-1}}(x_{t-1}, v_{t-1})\|^2} \nonumber.
	\end{align}
	The desired result follows by taking the square on both sides of the above inequality and using the fact that $(a+b)^2 \le 2a^2+2b^2$.
\end{proof}

We also need the following lemma, which was established as Lemma 1 and Proposition 1 in \cite{Ghadimi2016}.
\begin{lemma}[Lemma 1 and Proposition 1, \cite{Ghadimi2016}]\label{aux: 4}
	Let $g$ be a proper and closed convex function. Then, for all $u, v, x\in \mathbb{R}^d$ and $\eta>0$, the following statements hold:
	\begin{align*}
		&\inner{u}{G_{\eta}(x,u)} \ge \|G_{\eta}(x,u)\|^2 + \frac{1}{\eta} \big(g(\mathrm{prox}_{\eta g}(x-\eta u)) - g(x) \big), \\
		&\|G_{\eta}(x,u) - G_{\eta}(x,v)\| \le \|u-v\|.
	\end{align*}
\end{lemma}



\section{Proof of \Cref{thm: ProxSpiderM}}
Consider any iteration $k$ of the algorithm. By smoothness of $f$, we obtain that
\begin{align}
f(x_k) &\le f(x_{k-1}) + \inner{\nabla f(x_{k-1})}{x_k - x_{k-1}} + \frac{L}{2}\|x_k - x_{k-1}\|^2 \nonumber \\
&= f(x_{k-1}) + \inner{\nabla f(x_{k-1})}{- \lambda_{k-1} G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})} + \frac{L\lambda_{k-1}^2}{2}\|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 \nonumber \\
&= f(x_{k-1}) - \lambda_{k-1} \inner{\nabla f(x_{k-1})-v_{k-1}}{G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})} -  \lambda_{k-1} \inner{v_{k-1}}{G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})} \nonumber\\
&\quad+ \frac{L\lambda_{k-1}^2}{2}\|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 \nonumber\\
&\overset{(i)}{\le} f(x_{k-1}) - \lambda_{k-1} \inner{\nabla f(x_{k-1})-v_{k-1}}{G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})} -  \lambda_{k-1} \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2  \nonumber\\ 
\displaybreak
&\quad - \big(g(\mathrm{prox}_{\lambda_{k-1} g}(x_{k-1}-\lambda_{k-1} v_{k-1})) - g(x_{k-1}) \big) + \frac{L\lambda_{k-1}^2}{2}\|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 \nonumber\\
&= f(x_{k-1}) - \lambda_{k-1} \inner{\nabla f(x_{k-1})-v_{k-1}}{G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})} -  \lambda_{k-1} \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2  \nonumber\\ 
&\quad - \big(g(x_k) - g(x_{k-1}) \big) + \frac{L\lambda_{k-1}^2}{2}\|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2, \nonumber
\end{align}
where (i) follows from \Cref{aux: 4}. Rearranging the above inequality and using Cauchy-Swartz inequality yields that
\begin{align}
	F(x_k) \le  F(x_{k-1}) - \lambda_{k-1}(1-\frac{L\lambda_{k-1}}{2}) \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 + \lambda_{k-1} \|\nabla f(x_{k-1})-v_{k-1}\| \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|. \label{eq: 15}
\end{align}

Note that
\begin{align}
\|\nabla f(x_{k-1}) - v_{k-1}\| &\le \|\nabla f(x_{k-1}) - \nabla f(z_{k-1})\| + \|\nabla f(z_{k-1}) - v_{k-1}\| \nonumber \\
&\overset{(i)}{\le} L\|x_{k-1} - z_{k-1}\| + \|\nabla f(z_{k-1}) - v_{k-1}\| \nonumber \\
&\overset{(ii)}{\le} L(1-\alpha_k) \|y_{k-1} - x_{k-1}\| + \|\nabla f(z_{k-1}) - v_{k-1}\| \nonumber,
\end{align}
where (i) uses the Lipschitz continuity of $\nabla f$ and (ii) follows from the update rule of the momentum scheme. Substituting the above inequality into \cref{eq: 15} yields that
\begin{align}
F(x_k) &\le F(x_{k-1}) - \lambda_{k-1}(1-\frac{L\lambda_{k-1}}{2})\|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 + L\lambda_{k-1}(1-\alpha_k) \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|\|y_{k-1} - x_{k-1}\| \nonumber\\
&\quad + \lambda_{k-1} \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|\|\nabla f(z_{k-1}) - v_{k-1}\| \nonumber \\
&\le F(x_{k-1}) - \lambda_{k-1}(1-\frac{L\lambda_{k-1}}{2})\|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 + \frac{L\lambda_{k-1}^2}{2} \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 + \frac{L(1-\alpha_k)^2}{2}\|y_{k-1} - x_{k-1}\|^2 \nonumber\\
&\qquad+ \frac{\lambda_{k-1}}{2} \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 + \frac{\lambda_{k-1}}{2}\|\nabla f(z_{k-1}) - v_{k-1}\|^2 \nonumber \\
&= F(x_{k-1}) - \lambda_{k-1}(\frac{1}{2}-L\lambda_{k-1}) \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 + \frac{L(1-\alpha_k)^2}{2}\|y_{k-1} - x_{k-1}\|^2 + \frac{\lambda_{k-1}}{2}\|\nabla f(z_{k-1}) - v_{k-1}\|^2 \nonumber\\
&\le  F(x_{k-1}) - \lambda_{k-1}(\frac{1}{2}-L\lambda_{k-1}) \|G_{\lambda_{k-1}}(x_{k-1}, v_{k-1})\|^2 + \frac{L\Gamma_{k-1}}{2}\sum_{t=1}^{k-1} \frac{\lambda_{t-1} - \beta_{t-1}}{\alpha_t\Gamma_t} \|G_{\lambda_{t-1}}(x_{t-1}, v_{t-1})\|^2 \nonumber\\
&\quad+ \frac{\lambda_{k-1}}{2}\|\nabla f(z_{k-1}) - v_{k-1}\|^2, \nonumber
\end{align}
where the last inequality uses item 2 of \Cref{aux: 3} and the fact that $0<\alpha_k <1$.
Telescoping the above inequality over $k$ from $1$ to $K$ yields that
\begin{align}
F(x_{K}) &\le F(x_{0}) - \sum_{k=0}^{K-1} \lambda_k (\frac{1}{2}-L\lambda_k) \|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \sum_{k=0}^{K-1} \frac{L\Gamma_{k}}{2}\sum_{t=0}^{k-1} \frac{(\lambda_{t} - \beta_{t})^2}{\Gamma_{t+1}\alpha_{t+1}}  \|G_{\lambda_{t}}(x_{t}, v_{t})\|^2 + \sum_{k=0}^{K-1} \frac{\lambda_k}{2}\|\nabla f(z_{k}) - v_k\|^2 \nonumber \\
&= F(x_{0}) - \sum_{k=0}^{K-1} \lambda_k (\frac{1}{2}-L\lambda_k) \|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \frac{L}{2} \sum_{k=0}^{K-1} \frac{(\lambda_k - \beta_k)^2}{\Gamma_{k+1}\alpha_{k+1}} \|G_{\lambda_{k}}(x_{k}, v_{k})\|^2(\sum_{t=k}^{K-1} \Gamma_{t})  \nonumber\\
&\quad+ \sum_{k=0}^{K-1} \frac{\lambda_k}{2}\|\nabla f(z_{k}) - v_k\|^2, \label{eq: 30}
\end{align}
where we have exchanged the order of summation in the second equality. Furthermore, note that $\sum_{t=k}^{K-1} \Gamma_{t} = 2\sum_{t=k}^{K-1} \frac{1}{t} - \frac{1}{t+1} \le \frac{2}{k}$. Then, substituting this bound into the above inequality and taking expectation on both sides yield that
\begin{align}
\mathbb{E}[F(x_{K})] &\le F(x_{0}) - \sum_{k=0}^{K-1} \lambda_k (\frac{1}{2}-L\lambda_k) \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \frac{L}{2} \sum_{k=0}^{K-1} \frac{2(\lambda_k - \beta_k)^2}{k\Gamma_{k+1}\alpha_{k+1}} \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2  \nonumber\\
&\quad+ \sum_{k=0}^{K-1} \frac{\lambda_k}{2} \mathbb{E}\|\nabla f(z_{k}) - v_k\|^2. \label{eq: 16}
\end{align}

Next, we bound the term $\mathbb{E}\|\nabla f(z_{k}) - v_k\|^2$ in the above inequality. By \Cref{aux: 1} we obtain that
\begin{align}
\mathbb{E}\|\nabla f(z_{k}) - v_k\|^2 &\le \sum_{i=(\tau(k)-1)q}^{k-1}\frac{L^2}{|\xi_i|} \mathbb{E}\|z_{i+1} - z_{i}\|^2 \nonumber \\
&\le \sum_{i=(\tau(k)-1)q}^{k-1}\frac{L^2}{|\xi_i|} \big[2\beta_i^2\|G_{\lambda_{i}}(x_{i}, v_{i})\|^2 + 2\alpha_{i+2}^2 \Gamma_{i+1}\sum_{t=0}^{i} \frac{(\lambda_{t} - \beta_{t})^2}{\alpha_{t+1}\Gamma_{t+1}} \|G_{\lambda_{t}}(x_{t}, v_{t})\|^2 \big], \label{eq: 17}
\end{align}
where the last inequality uses item 3 of \Cref{aux: 3}. Substituting \cref{eq: 17} into \cref{eq: 16} and simplifying yield that
\begin{align}
\mathbb{E}[F(x_{K})] &\le F(x_{0}) - \sum_{k=0}^{K-1} \Big[\lambda_k (\frac{1}{2}-L\lambda_k) - \frac{L(\lambda_k - \beta_k)^2}{k\Gamma_{k+1}\alpha_{k+1}}\Big] \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 \nonumber\\
&\quad + \underbrace{\sum_{k=0}^{K-1} \frac{\lambda_k}{2} \mathbb{E}\bigg[\sum_{i=(\tau(k)-1)q}^{k-1}\frac{L^2}{|\xi_i|} \bigg[2\beta_i^2\|G_{\lambda_{i}}(x_{i}, v_{i})\|^2 + 2\alpha_{i+2}^2 \Gamma_{i+1}\sum_{t=0}^i \frac{(\lambda_t - \beta_t)^2}{\alpha_{t+1}\Gamma_{t+1}} \|G_{\lambda_{t}}(x_{t}, v_{t})\|^2 \bigg] \bigg]}_{T}. \label{eq: 18}
\end{align}
Before we proceed the proof, we first specify the choices of all the parameters. Specifically, we choose a constant mini-batch size $|\xi_k|\equiv |\xi|$, a constant $q=|\xi|$, a constant $\beta_k \equiv \beta>0$, $\lambda_k \in [\beta, (1+\alpha_{k+1})\beta]$. Based on these parameter settings, the term $T$ in the above inequality can be bounded as follows.
\begin{align}
T &\overset{(i)}{\le} \sum_{k=0}^{K-1} \frac{\lambda_k}{2} \mathbb{E}\bigg[\sum_{i=(\tau(k)-1)q}^{\tau(k)q-1}\frac{L^2}{|\xi_i|} \bigg[2\beta_i^2\|G_{\lambda_{i}}(x_{i}, v_{i})\|^2 + 2\alpha_{i+2}^2 \Gamma_{i+1}\sum_{t=0}^{k-1} \frac{(\lambda_t - \beta_t)^2}{\alpha_{t+1}\Gamma_{t+1}} \|G_{\lambda_{t}}(x_{t}, v_{t})\|^2 \bigg] \bigg] \nonumber\\
&\overset{(ii)}{\le} \sum_{k=0}^{K-1} \frac{\lambda_k L^2q\beta^2}{|\xi|}\mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \sum_{k=0}^{K-1} \frac{2\lambda_kL^2}{|\xi|[(\tau(k)-1)q+1]^3} \sum_{t=0}^{k-1}\frac{(\lambda_t - \beta_t)^2}{\alpha_{t+1}\Gamma_{t+1}}\mathbb{E}\|G_{\lambda_{t}}(x_{t}, v_{t})\|^2  \nonumber\\
&\overset{(iii)}{\le} \sum_{k=0}^{K-1} \lambda_k L^2\beta^2 \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \frac{2L^2\beta^2}{|\xi|} \sum_{k=0}^{K-1}  \frac{\alpha_{k+1}}{\Gamma_{k+1}} \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 (\sum_{t=k}^{K-1} \frac{\lambda_k}{[(\tau(t)-1)q+1]^3})   \nonumber\\
&\overset{(iv)}{\le} \sum_{k=0}^{K-1} \lambda_k L^2\beta^2 \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \frac{4L^2\beta^3}{|\xi|} \sum_{k=0}^{K-1} (k+1) \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 (\sum_{t=(\tau(k)-1)q}^{\tau(K)q} \frac{1}{[(\tau(t)-1)q+1]^3})   \nonumber\\
&= \sum_{k=0}^{K-1} \lambda_k L^2\beta^2 \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \frac{4L^2\beta^3}{|\xi|} \sum_{k=0}^{K-1} (k+1) \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 (\sum_{t=\tau(k)-1}^{\tau(K)} \frac{q}{(tq+1)^3})  \nonumber\\
&\le \sum_{k=0}^{K-1} \lambda_k L^2\beta^2 \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \frac{2L^2\beta^3}{q} \sum_{k=0}^{K-1} (k+1) \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 \frac{1}{[(\tau(k)-1)q+1]^2}   \nonumber \\
&\overset{(v)}{\le} \sum_{k=0}^{K-1} \lambda_k L^2\beta^2 \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + 2L^2\beta^3 \sum_{k=0}^{K-1} \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 \frac{\tau(k)}{[(\tau(k)-1)q+1]^2} \nonumber\\
&\le \sum_{k=0}^{K-1} \lambda_k L^2\beta^2 \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + 2L^2\beta^3 \sum_{k=0}^{K-1} \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2, \label{eq: 19}
\end{align}
where (i) follows from the facts that $i\le k-1$ and $k-1\le \tau(k)q-1$, (ii) uses the fact that $\sum_{i=(\tau(k)-1)q}^{\tau(k)q-1} \alpha_{i+2}^2\Gamma_{i+1} \le \frac{2}{(\tau(k)-1)q+1)^3}$, (iii) uses the parameter settings $q=|\xi|$ and $\lambda_t-\beta_t \le \alpha_t\beta$, (iv) uses the facts that $\lambda_k\le 2\beta$ and $(\tau(k)-1)q \le k\le \tau(k)q$ and (v) uses the fact that $k \le \tau(k)q-1$. Substituting the above inequality into \cref{eq: 18} and simplifying, we obtain that
\begin{align}
\mathbb{E}[F(x_{K})] &\le F(x_{0}) - \sum_{k=0}^{K-1} \Big[\lambda_k (\frac{1}{2}-L\lambda_k - L^2\beta^2) - \frac{L(\lambda_k - \beta_k)^2}{k\Gamma_{k+1}\alpha_{k+1}} -2L^2\beta^3 \Big] \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 \label{eq: 31}\\
&\le F(x_{0}) - \sum_{k=0}^{K-1} \Big[\beta (\frac{1}{2}-2L\beta - L^2\beta^2) - L\beta^2 -2L^2\beta^3 \Big] \mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2. \label{eq: 32}
\end{align}
Choosing $\beta \le \frac{1}{8L}$, the above inequality further implies that
\begin{align}
\mathbb{E} [F(x_{K})] &\le F(x_{0}) - \sum_{k=0}^{K-1} \frac{\beta}{16}\mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 . \label{eq: 27}
\end{align}
Then, it follows that $\frac{1}{K}\sum_{k=0}^{K-1}\mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 \le 16(F(x_0) - F^*)/(K\beta)$. Next, we bound the term $\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\|^2$, where $\zeta$ is selected uniformly at random from $\{0,\ldots,K-1\}$. Observe that
\begin{align}
\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\|^2  &= \mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta})) -G_{\lambda_{\zeta}}(z_{\zeta}, v_{\zeta}) + G_{\lambda_{\zeta}}(z_{\zeta}, v_\zeta)\|^2 \nonumber\\
&\le 2\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta})) -G_{\lambda_{\zeta}}(z_{\zeta}, v_{\zeta})\|^2 + 2\mathbb{E}  \| G_{\lambda_{\zeta}}(z_{\zeta}, v_\zeta)\|^2 \nonumber\\
&\overset{(i)}{\le} 2\mathbb{E}  \|\nabla f(z_{\zeta}) - v_{\zeta}\|^2 + 2\mathbb{E}  \| G_{\lambda_{\zeta}}(z_{\zeta}, v_\zeta) - G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta) + G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 \nonumber\\
&\le 2\mathbb{E}  \|\nabla f(z_{\zeta}) - v_{\zeta}\|^2 + 4\mathbb{E}  \| G_{\lambda_{\zeta}}(z_{\zeta}, v_\zeta) - G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2  + 4\mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 \nonumber\\
&\le 2\mathbb{E}  \|\nabla f(z_{\zeta}) - v_{\zeta}\|^2 + 4\mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 \nonumber\\
&\quad+ \frac{4}{\lambda_{\zeta}^2}\mathbb{E}  \| z_{\zeta} - x_{\zeta} + \mathrm{prox}_{\lambda_{\zeta}g}(x_\zeta - \lambda_{\zeta}v_\zeta) - \mathrm{prox}_{\lambda_{\zeta}g}(z_\zeta - \lambda_{\zeta}v_\zeta)\|^2   \nonumber\\
&\le 2\mathbb{E}  \|\nabla f(z_{\zeta}) - v_{\zeta}\|^2 + 4\mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 \nonumber\\
&\quad+ \frac{8}{\lambda_{\zeta}^2}\mathbb{E}  \| z_{\zeta} - x_{\zeta}\|^2 +\frac{8}{\lambda_{\zeta}^2}\mathbb{E}  \|\mathrm{prox}_{\lambda_{\zeta}g}(x_\zeta - \lambda_{\zeta}v_\zeta) - \mathrm{prox}_{\lambda_{\zeta}g}(z_\zeta - \lambda_{\zeta}v_\zeta)\|^2   \nonumber\\
&\overset{(ii)}{\le} 2\mathbb{E}  \|\nabla f(z_{\zeta}) - v_{\zeta}\|^2 + 4\mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 + \frac{8}{\lambda_{\zeta}^2}\mathbb{E}  \| z_{\zeta} - x_{\zeta}\|^2 +\frac{8}{\lambda_{\zeta}^2}\mathbb{E}  \|z_{\zeta} - x_{\zeta}\|^2   \nonumber\\
&\overset{(iii)}{\le} 2\mathbb{E}  \|\nabla f(z_{\zeta}) - v_{\zeta}\|^2 + 4\mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 + \frac{16}{\lambda_{\zeta}^2}\mathbb{E}  \| y_{\zeta} - x_{\zeta}\|^2 \label{eq: 29}
\end{align}
where (i) uses the non-expansiveness property of the operator $G$ in \Cref{aux: 4}, (ii) follows from the non-expansiveness of the proximal operator, and (iii) uses the update rule and the fact that $0<\alpha_k<1$.

Next, we bound the three terms on the right hand side of the above inequality separately. First, note that
\begin{align*}
\mathbb{E} \|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2  = \frac{1}{K }\sum_{k=0}^{K-1} \mathbb{E} \|G_{\lambda_{k}}(x_{k}, v_k)\|^2 \le \frac{16(F(x_0) - F^*)}{K\beta}. 
\end{align*}
Second, note that \cref{eq: 17} implies that
\begin{align*}
\mathbb{E}  \|\nabla f(z_\zeta)-v_\zeta\|^2  &\le \mathbb{E}\sum_{i=(\tau(\zeta)-1)q}^{\zeta-1}\frac{L^2}{|\xi_i|} \big[2\beta_i^2\|G_{\lambda_{i}}(x_{i}, v_i)\|^2 + 2\alpha_{i+2}^2 \Gamma_{i+1}\sum_{t=0}^{i} \frac{(\lambda_{t} - \beta_{t})^2}{\alpha_{t+1}\Gamma_{t+1}} \|G_{\lambda_{t}}(x_{t}, v_t)\|^2 \big] \nonumber\\
&\le \frac{2L^2\beta^2}{|\xi|} \mathbb{E} \bigg(\sum_{i=(\tau(\zeta)-1)q}^{\tau(\zeta)q-1} \|G_{\lambda_{i}}(x_{i}, v_i)\|^2\bigg) + \frac{L^2}{|\xi|} \mathbb{E} \bigg(\sum_{i=(\tau(\zeta)-1)q}^{\zeta-1} 2\alpha_{i+2}^2 \Gamma_{i+1}\sum_{t=0}^{i} \frac{(\lambda_{t} - \beta_{t})^2}{\alpha_{t+1}\Gamma_{t+1}} \|G_{\lambda_{t}}(x_{t}, v_t)\|^2 \bigg) \nonumber\\
\displaybreak
&\le \frac{2L^2\beta^2}{|\xi|} \frac{1}{K} \sum_{\zeta=0}^{K-1} \bigg(\sum_{i=(\tau(\zeta)-1)q}^{\tau(\zeta)q-1} \mathbb{E}\|G_{\lambda_{i}}(x_{i}, v_i)\|^2\bigg) \nonumber\\
&\quad+ \frac{L^2 \beta^2}{|\xi|} \frac{1}{K} \sum_{\zeta=0}^{K-1} \bigg(\sum_{i=(\tau(\zeta)-1)q}^{\tau(\zeta)q-1} 2\alpha_{i+2}^2 \Gamma_{i+1}\sum_{t=0}^{\zeta-1} (t+1) \mathbb{E}\|G_{\lambda_{t}}(x_{t}, v_t)\|^2 \bigg) \nonumber\\
&\le \frac{2L^2\beta^2 q}{|\xi|} \frac{1}{K} \sum_{\zeta=0}^{K-1} \mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 + \frac{L^2 \beta^2}{|\xi|} \frac{1}{K} \sum_{\zeta=0}^{K-1} \bigg(\frac{4}{[(\tau(\zeta)-1)q+1]^3}\sum_{t=0}^{\zeta-1} (t+1) \mathbb{E}\|G_{\lambda_{t}}(x_{t}, v_t)\|^2 \bigg) \nonumber\\
&\le 2L^2\beta^2 \bigg(\frac{1}{K} \sum_{\zeta=0}^{K-1} \mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2\bigg) + \frac{L^2 \beta^2}{|\xi|} \frac{1}{K} \sum_{\zeta=0}^{K-1} (\zeta+1) \mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 \sum_{t=\zeta}^{K-1} \frac{4}{[\tau(t)-1)q+1]^3} \nonumber\\
&\le 2L^2\beta^2 \bigg(\frac{1}{K} \sum_{\zeta=0}^{K-1} \mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2\bigg) + L^2 \beta^2 \frac{1}{K} \sum_{\zeta=0}^{K-1} \mathbb{E}\|G_{\lambda_{\zeta}}(x_{\zeta}, v_\zeta)\|^2 \frac{2\tau(\zeta)}{[\tau(\zeta)-1)q+1]^2} \nonumber\\
&\le 3L^2\beta \frac{16(F(x_0) - F^*)}{K}, \nonumber
\end{align*} 
where we have used the fact that $\zeta$ is sampled uniformly from $0,...,K-1$ at random. 

Third, note that by item 2 of \Cref{aux: 3}, we know that
\begin{align}
	\mathbb{E}  \| y_{\zeta} - x_{\zeta}\|^2 &\le \mathbb{E} \bigg(\Gamma_\zeta\sum_{t=0}^{\zeta-1} \frac{\lambda_{t} - \beta_{t}}{\alpha_{t+1}\Gamma_{t+1}}  \|G_{\lambda_{t}}(x_{t}, v_{t})\|^2\bigg) \nonumber\\
	&\le \frac{1}{K} \sum_{\zeta=0}^{K-1} \Gamma_\zeta\sum_{t=0}^{\zeta-1} \frac{\lambda_{t} - \beta_{t}}{\alpha_{t+1}\Gamma_{t+1}} \mathbb{E}  \|G_{\lambda_{t}}(x_{t}, v_{t})\|^2 \nonumber\\
	&\le \frac{\beta^2}{K} \sum_{\zeta=0}^{K-1} \Gamma_\zeta\sum_{t=0}^{\zeta-1} (t+1) \mathbb{E}  \|G_{\lambda_{t}}(x_{t}, v_{t})\|^2 \nonumber\\
	&= \frac{\beta^2}{K} \sum_{\zeta=0}^{K-1} (\zeta+1) \mathbb{E}  \|G_{\lambda_{\zeta}}(x_{\zeta}, v_{\zeta})\|^2 \bigg(\sum_{t=\zeta+1}^{K-1}\Gamma_t \bigg) \nonumber\\
	&\le \frac{\beta^2}{K} \sum_{\zeta=0}^{K-1} \mathbb{E}  \|G_{\lambda_{\zeta}}(x_{\zeta}, v_{\zeta})\|^2.
\end{align}

Combining the above three inequalities and note that $L\beta = \Theta(1)$ and $\frac{\beta}{\lambda_k} \le 1$, we finally obtain that
\begin{align}
\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\|^2  \le \Theta\bigg(\frac{L(F(x_0) - F^*)}{K} \bigg) . \label{eq: 20}
\end{align}
This further implies that
\begin{align*}
\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\| \le \sqrt{\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\|^2} \le \Theta\bigg(\sqrt{\frac{L(F(x_0) - F^*)}{K}}\bigg). 
\end{align*}
Setting the right hand side of the above inequality to be bounded by $\epsilon$, we obtain that $K \ge \Theta\bigg(\frac{L(F(x_0) - F^*)}{\epsilon^2} \bigg)$. Then, the total number of stochastic gradient calls is bounded by $(K+q)\frac{n}{q} + K|\xi| \le \Theta(n+\sqrt{n}\epsilon^{-2})$.


\section{Proof of \Cref{thm: ProxSpiderP}}
The convergence proof of Proximal SPIDER-M with both epochwise-diminishing momentum and epochwise restart momentum follow from that of Proximal SPIDER-M, and therefore we only describe the key steps to adapt the proof.  


We first prove the result of Proximal SPIDER-M with epochwise-diminishing momentum. Under the epochwise-diminishing momentum scheme, the momentum coefficient is set to be $\alpha_{k} = \frac{2}{\ceil[]{k/q}+1}$. Consequently, we have $\Gamma_{k} = \frac{2}{\ceil[]{k/q}(\ceil[]{k/q}+1)}$. First, one can check that \cref{eq: 30} still holds, and now we have $\sum_{t=k}^{K-1} \Gamma_{t} \le \frac{2}{\ceil[]{k/q}}$. Then, we follow the steps that bound the accumulation error term $T$ in \cref{eq: 18}. In the derivation of (ii), we now have that $\sum_{i=(\tau(k)-1)q}^{\tau(k)q-1} \alpha_{i+2}^2\Gamma_{i+1} \le \frac{2}{\tau(k)^3}$. Substituting this new bound into (ii) and noting that in (iii) we now have $\frac{\alpha_{k+1}}{\Gamma_{k+1}} = (\ceil[]{k/q}+1)$, one can follow the subsequent steps and show that the upper bound for T in \cref{eq: 19} still holds. Moreover, in \cref{eq: 31} we should replace $\frac{L(\lambda_k - \beta_k)^2}{k\Gamma_{k+1}\alpha_{k+1}}$ with $\frac{L(\lambda_k - \beta_k)^2}{\ceil[]{k/q}\Gamma_{k+1}\alpha_{k+1}}$, and consequently \cref{eq: 32} is still valid. Then, one can follow the same analysis and show that \cref{eq: 27} is still valid. In summary, the convergence rate and the corresponding oracle complexity remain in the same order.


The convergence proof of Proximal SPIDER-M with periodic restart follows from that of Proximal SPIDER-M. The core idea is to apply the result of Proximal SPIDER-M to each restart period. 
Specifically, consider the iterations $k=0,1,...,q-2$. As no restart is performed within these iterations, we can apply the result in \cref{eq: 20} (note that $F^*$ is the relaxation of $F(x_K)$) obtained from the analysis of Proximal SPIDER-M and conclude that
\begin{align}
\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\|^2 \le \Theta\bigg(\frac{L(F(x_0) - \mathbb{E}[F(x_{q-1})])}{q-1} \bigg), ~\text{where}~ \zeta \overset{\text{Unif}}{\sim}\{0,...,q-2\}.
\end{align}
Due to the periodic restart, the above bound also holds similarly for the iterations $k=tq,tq+1,...,(t+1)q-2$ for any $t\in \mathbb{N}$, which yields that
\begin{align}
\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\|^2 \le \Theta\bigg(\frac{L(F(x_{tq}) - \mathbb{E}[F(x_{(t+1)q-1})])}{q-1} \bigg), ~\text{where}~ \zeta \overset{\text{Unif}}{\sim}\{tq,...,(t+1)q-2\}. \label{eq: 21}
\end{align}
Next, consider running the algorithm with restart for iterations $k=0,...,K-1$, and the output index $\zeta$ is selected from $\{k: 0\le k\le K-1, \textrm{mod}(k,q-1)\ne0 \}$ uniformly at random. Let $T = \ceil[\Big]{\frac{K}{q-1}}$. Then, we can obtain the following estimate
\begin{align}
\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\|^2 &\le \frac{1}{K-T} \sum_{t=0}^{T} \sum_{k=tq}^{(t+1)q-2} \mathbb{E}  \|G_{\lambda_{k}}(z_{k}, \nabla f(z_{k}))\|^2 \nonumber\\
&\overset{(i)}{\le} \Theta \bigg(\frac{1}{K-T} \sum_{t=0}^{T} L\mathbb{E}(F(x_{tq}) - F(x_{(t+1)q-1})) \bigg) \nonumber\\
&\overset{(ii)}{\le} \Theta \bigg(\frac{L(F(x_{0}) - F^*)}{K} \bigg), \nonumber
\end{align}
where (i) uses the results inductively derived from \cref{eq: 21} and (ii) uses the fact that $x_{(t+1)q-1} = x_{(t+1)q}$ due to restart. 

Therefore, it follows that $\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\| \le \epsilon$ whenever $K \ge \Theta \bigg(\frac{L(F(x_{0}) - F^*)}{\epsilon^2} \bigg)$, and the total number of stochastic gradient calls is in the order of $\Theta(n+\sqrt{n}\epsilon^{-2})$. 

\section{Proof of \Cref{thm: ProxSpiderO}}
Note that when $\textrm{mod}(k,q)=0$, the Online Proximal SPIDER-M samples $\xi_1$ data points to estimate the gradient, and we obtain the following variance bound based on \Cref{assum: variance}.
\begin{align}
	\mathbb{E} \|v_k - \nabla f(x_k)\|^2 &= \mathbb{E} \bigg\| \frac{1}{|\xi_1|}\sum_{i = 1}^{|\xi_1|} \nabla \ell_{u_i}(x_k) - \nabla f(x_k) \bigg\|^2  \le \frac{1}{|\xi_1|^2} \sum_{i =1}^{|\xi_1|} \mathbb{E}\left\|   \nabla \ell_{u_i}(x_k) - \nabla f(x_k)\right\|^2 \le \frac{\sigma^2}{|\xi_1|}.
\end{align}
By telescoping \Cref{lemma: Zhang} and using the above bound, we obtain the following lemma.
\begin{lemma}\label{aux: 5}
	Under Assumptions \ref{assum: f} and \ref{assum: variance}, the estimation of gradient $v_k$ constructed by Online Proximal SPIDER-M satisfies that for all $k\in \mathbb{N}$,
	\begin{align}
	\mathbb{E} \|v_k - \nabla f(z_k)\|^2 \le \sum_{i=(\tau(k)-1)q}^{k-1}\frac{L^2}{|\xi_i|} \mathbb{E}\|z_{i+1} - z_{i}\|^2 + \frac{\sigma^2}{|\xi_1|}. \label{eq: var online}
	\end{align}
\end{lemma}

Then, one can check that \cref{eq: 16} still holds in the online case. Therefore, we can apply the bound in \Cref{aux: 5} to \cref{eq: 16} and follow the proof of \cref{eq: 27}. One can check that there is an additional term $\sum_{k=0}^{K-1} \frac{\lambda_{k}\sigma^2}{2|\xi_1|}$ in the online case, and we obtain the following bound. 
\begin{align}
\mathbb{E} [F(x_{K})] &\le F(x_{0}) - \sum_{k=0}^{K-1} \frac{\beta}{16}\mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \sum_{k=0}^{K-1} \frac{\lambda_{k}\sigma^2}{2|\xi_1|} \nonumber\\
&\le F(x_{0}) - \sum_{k=0}^{K-1} \frac{\beta}{16}\mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 + \frac{K\beta\sigma^2}{|\xi_1|}. \label{eq: 28}
\end{align}
Then, it follows that $\frac{1}{K}\sum_{k=0}^{K-1}\mathbb{E}\|G_{\lambda_{k}}(x_{k}, v_{k})\|^2 \le 16(F(x_0) - F^*)/(K\beta) + \frac{16\sigma^2}{|\xi_1|}$. One can check that \cref{eq: 29} still holds, and we only need to update the bound for the term $\mathbb{E}  \|\nabla f(z_{\zeta}) - v_{\zeta}\|^2$ as follows
\begin{align}
	\mathbb{E}  \|\nabla f(z_{\zeta}) - v_{\zeta}\|^2 \le 3L^2\beta \frac{16(F(x_0) - F^*)}{K} + \frac{\sigma^2}{|\xi_1|}.
\end{align}
Then, we finally obtain that 
\begin{align}
\mathbb{E}  \|G_{\lambda_{\zeta}}(z_{\zeta}, \nabla f(z_{\zeta}))\|^2  \le \Theta\bigg(\frac{L(F(x_0) - F^*)}{K} + \frac{\sigma^2}{|\xi_1|}\bigg).
\end{align}
To make the right hand side be smaller than $\epsilon^2$, we can set $K\ge \frac{2L(F(x_0) - F^*)}{\epsilon^2}$ and $|\xi_1|\ge \frac{2\sigma^2}{\epsilon^2}$. This proves the desired iteration complexity. On the other hand, the total number of stochastic gradient oracle calls is at most $(K+q)\frac{|\xi_1|}{q} + K|\xi_2|$. By setting $q=|\xi_2|=\sqrt{|\xi_1|}$, we obtain the total oracle complexity as $\Theta(\epsilon^{-3})$.

\section{Proof of \Cref{thm: ProxSpiderO-other}}
The proof follows exactly from that of \Cref{thm: ProxSpiderP} (the same treatment of the momentum schemes apply). 
















==> introduction_oldv1.tex <==
\section{Introduction}
In this paper, we study  the following nonconvex and nonsmooth composite optimization problem
\begin{align}\label{objecP}
\min_{x\in \mathbb{R}^d} \Psi(x):=f(x)+h(x), \tag{P}
\end{align}
where $h(x)$ is a simple but nonsmooth convex function and $f(x)$ has the following finite-sum form 
\begin{align}
f(x)=\frac{1}{n}\sum_{i=1}^n f_i(x),
\end{align}
where $l_i(x), i=1,...,n$ are $n$ individual nonconvex and smooth functions. 
 Such a problem has attracted a lot attention in many regularized machine learning problems, e.g., egularized empirical risk minimization problems~\cite{??}.  To handle the non-smoothness  of the function $h(x)$, one natural way is to conduct the following proximal update 
\begin{align}
x_{k+1} = \mathrm{prox}_{\eta h}(x_k - \eta v_k)
\end{align}
at the $k^{th}$ iteration, where the proximal mapping is given by 
\begin{align}\label{pmap}
	\text{(Proximal mapping):}~\mathrm{prox}_{\eta h}(x):= \arg\min_{u\in\mathbb{R}^d} \Big\{h(u) + \frac{1}{2\eta}\|u-x\|^2\Big\}.  
\end{align}
and $v_k$ is the stochastic gradient estimation of $\nabla f(x_k)$. Based on such a technique,  \cite{Ghadimi2016} proposed a proximal stochastic gradient decent (ProxSGD) by picking $v_k=\nabla \ell_{i_k}f(x_k)$ with $i_{k}$ chosen from $\{1,...,n\}$ uniformly at random, and proposed a proximal gradient decent (ProxGD) by choosing $v_k=\nabla f(x_k)$. Measured by the stochastic first-order (SFO) complexity that is the number of computation of stochastic gradients,  and the proximal oracle (PO) complexity that is the number of computation of proximal projections,  ProxSGD and ProxGD achieve a SFO complexity of $\mathcal{O}(\min\{n\epsilon^{-1}, \epsilon^{-2}\})$ and a PO complexity of $\mathcal{O}(\epsilon^{-1})$ to obtain a $\epsilon$-approximate first-order stationary point, i.e., $\mathbb{E}\|\nabla G_{\eta}(x)\|^2\leq \epsilon$, where $G_{\eta}(x)$ is the generalized gradient of function $\Psi(\cdot)$ at the point $x$. To accelerate the convergence rate, the stochastic variance reduced gradient (SVRG) based and the SAGA based proximal algorithms were proposed by \cite{Reddi2016,Allen_Zhu2017,Li2018} and achieved a SFO complexity of $\mathcal{O}(\min\{n^{2/3}\epsilon^{-1},\epsilon^{-5/3}\})$,  which improve the SFO complexity of ProxSGD and ProxGD by a factor of $\mathcal{O}(\min\{n^{1/3},\epsilon^{-1/3}\})$.  

 Recently,  \cite{Fang2018} proposed a new variance reduction technique named Spider for solving the finite-sum nonconvex optimization problem, i.e., the problem~\eqref{objecP} with $h(x)\equiv0$, which achieves a near-optimal gradient complexity to obtain an $\epsilon$-approximate first-order stationary point. Thus, one natural question is 
 \begin{align*}
 \textit{Can we further improve the SFO complexity of existing proximal algorithms by Spider?} 
\end{align*}
We answer this question affirmably  but by using a more practical variant of Spider, which we call as SpiderBoost. Compared with Spider, our developed SpiderBoost has two main advantages. First, SpiderBoost allows a much larger stepsize $\eta_k=\mathcal{O}(1/L)$ than the stepsize $\eta_k=\mathcal{O}(\epsilon/\left(L\|v_k\|\right)), \|v_k\|\geq \epsilon$ adopted by Spider without any theoretical performance loss. As a result, our SpiderBoost achieves significantly larger progress towards to the first-order stationary point than Spider especially in the initial optimization phase where $\|v_k\|$ is large, as demonstrated in our experiment.  Second, Spider  requires a extremely small per-iteration increment $\|x_{k+1}-x_k\|=\mathcal{O}(\epsilon/L)$, whereas  our SpiderBoost only needs $\|x_{k+1}-x_k\|$ to be $\mathcal{O}(1/L)$. Such a flexibility makes our SpiderBoost more easily extend to the proximal algorithm than Spider, as restricting the proximal projection within a $\mathcal{O}(\epsilon)$ region is challenging both in the theoretical analysis and the practical usage. % large increment  $\|x_{k+1}-x_k\|=\mathcal{O}(1/L)$, whereas SPIDER requires $x_{k+1}-x_{k}=\mathcal{O}(\epsilon/L)$.
%$\ell_i(\cdot): \mathbb{R}^d \rightarrow \mathbb{R}$ corresponds to the loss function on the $i$-th data sample and function $h$ denotes the regularizer that promotes desired structures to the solution based on our prior knowledge. Due to the big data trend, the demanding large data size $n$ makes it impossible to apply gradient descent method, which hiders the  efficiency of gradient descent (GD) and leads to  an overall gradient complexity of $O( n\epsilon^{-1})$ \citep{Nesterov2014} to obtain an $\epsilon$-approximate first-order stationary point. On the other hand, SGD is a possible candidate algorithm due to its low per-iteration sample complexity. However, its applicability is restricted by its notoriously slow convergence rate.

We generalize  the scheme of SpiderBoost for solving the composite problem~\eqref{objecP}, and propose Prox-SpiderBoost, which achieve a SFO complexity of $\mathcal{O}(\min\{n^{1/2}\epsilon^{-1},\epsilon^{-3/2}\})$ and a PO complexity of $\mathcal{O}(\epsilon^{-1})$. Such a SFO complexity improves the existing best results by a factor of $\mathcal{O}(\min\{n^{1/6},\epsilon^{-1/6}\})$. 
%We note that the previous studies mainly focus on the 
We further extend Prox-SpiderBoost  for solving the constrained composite optimization using the proximal mapping under a non-Euclidean geometry, i.e., by replacing the $\mathbb{R}^{d}$ in the problem~\eqref{objecP} by a convex constraint set $\mathcal{X}$, and the Euclidean distance $\|\cdot\|$ in~\eqref{pmap} by a generalized Bregman distance. Under certain conditions, we prove that the obtained algorithm achieves the same  SFO complexity and  PO complexity as Prox-SpiderBoost  for solving the unconstrained problem~\eqref{objecP}.


We  further revise our Prox-SpiderBoost for restricted strongly convex optimization, where the both objective functions $f$ and $g$ are restricted strongly convex (such a condition is more relaxed than the global strongly convexity condition, see section ? for its detailed definition). We show that Prox-SpiderBoost has an order-level $\mathcal{O}(n)$ improvement over ProxSVRG in the convergence rate under a standard choice of stepsize, and more importantly, it improves the oracle complexity of the existing variance reduction based algorithms without momentum acceleration (e.g., ProxSVRG, ProxSAGA) by a factor of $\mathcal{O}(\log c)$, where $c$ is a large number and has the order of $\Theta(n)$ for most well-conditioned problems.

We then study the performance of Prox-SpiderBoost for the online stochastic composite optimization problem, where the objective function $f(x)=\mathbb{E}_{\zeta} [\ell_{\zeta}(x)]$ over the underlying data distribution. Our results show that Prox-SpiderBoost still improves the existing best SFO complexity by a factor of $\epsilon^{-1/6}$. Such a complexity also holds for generalized constrained optimization under a non-Euclidean geometry. 
{\color{red} I did not separately write the online case}

\renewcommand{\arraystretch}{1.3} 
\definecolor{LightCyan}{rgb}{0.88,1,1}
\begin{table}[H] 
	\centering 
\resizebox{6.5in}{!}{	
	\begin{tabular}{clllcll} \toprule
		\multirow{2}{*}{Algorithms}& &\multirow{2}{*}{Stepsize $\eta$} &\multicolumn{2}{c}{Finite-Sum}       &\multicolumn{2}{c}{Online} \\ 
		\cmidrule{4-5}   \cmidrule{6-7} 
		&  & &\multicolumn{1}{c}{SFO} &\multicolumn{1}{c}{PO}    &\multicolumn{1}{c}{SFO} &\multicolumn{1}{c}{PO} \\   \midrule
%		ProxGD &\citep{Ghadimi2016}\footnotemark &$\mathcal{O}(L^{-1})$ &  $\mathcal{O}(n \epsilon^{-1} )$    & $\mathcal{O}( \epsilon^{-1} )$   & & \\ \midrule
		
		ProxSGD/ProxGD  &\citep{Ghadimi2016} &$\mathcal{O}(L^{-1})$  & $\mathcal{O}(n \epsilon^{-1} )$   &  $\mathcal{O}( \epsilon^{-1} )$ &$\mathcal{O}(\epsilon^{-2}  )$   &$\mathcal{O}( \epsilon^{-1} )$ \\ \midrule
		
		ProxSVRG/SAGA &\citep{Reddi2016} &$\mathcal{O}(L^{-1})$ &  $\mathcal{O}(n^{2/3} \epsilon^{-1}  )$    & $\mathcal{O}( \epsilon^{-1} )$  &N/A &N/A \\ \midrule
		Natasha1.5  &\citep{Allen_Zhu2017} &$\mathcal{O}(\epsilon^{4/3}L^{-2/3})$ &N/A &N/A    &  $\mathcal{O}(  \epsilon^{-5/3}  )$    & $\mathcal{O}( \epsilon^{-5/3} )$  \\ \midrule
		
		ProxSVRG$^\textbf{+}$ &\citep{Li2018} \footnotemark &$\mathcal{O}(L^{-1})$&$\mathcal{O}(n^{2/3}\epsilon^{-1})$& $\mathcal{O}(\epsilon^{-1})$ &   $\mathcal{O}(  \epsilon^{-5/3}  )$    & $\mathcal{O}( \epsilon^{-1} )$   \\  \midrule
		
		\belowrulesepcolor{LightCyan}   
		\rowcolor{LightCyan}
		ProxSPIDER$^\textbf{+}$ &(This Work) &$\mathcal{O}(L^{-1})$ & $\mathcal{O}(n^{1/2}\epsilon^{-1})$&  $\mathcal{O}(\epsilon^{-1})$ &    $\mathcal{O}(  \epsilon^{-3/2}  )$    & $\mathcal{O}( \epsilon^{-1} )$  \\   \aboverulesepcolor{LightCyan}  \bottomrule
	\end{tabular} 
}
	\vspace{2mm}
	\caption{Comparable results on gradient complexity and proximal cost for nonsmooth nonconvex  optimization.} \label{comparison_nonsmooth}
\end{table} 
%\footnotetext[4]{We note that for deterministic algorithms, the online setting does not exist.} 
\footnotetext[5]{This paper has a detail discussion about the choice of outer loop batch size, we only present the best result of it.} 

------------------------------------------------------------------------------------ (zhe "s )

 To overcome such issue and reduce the dependent on $n$, stochastic gradient descent method  (SGD) is proposed, which calculates one gradient per iteration and yields an overall gradient complexity of $O(\epsilon^{-2})$ \citep{Ghadimi2016}, which is also its convergence rate since it only calculates one gradient per iteration. SGD efficiently drops the dependent on $n$, but the convergence rate is slower as compared to $O(\epsilon^{-1})$ convergence rate of GD and is more rely on the target accuracy $\epsilon$. Moreover, the vanilla SGD can only converge to the neighbor of first-order stationary points instead of the exact stationary points. The inexact convergence issue can be eliminated by diminishing the step-size \citep{Bottou2018} or choose a sufficient large batch size in each iteration.  
 
 However, the slow convergence issue still hiders the application of stochastic gradient-based method in various situation, especially for   machine learning problems that requires high accuracy solutions. Fortunately, this issue has been identified as variance issue, which caused by the inexact estimation of using stochastic gradient to estimate the full gradient. Thus, various variance reduction methods have been proposed to reduce the variance of the gradient estimator  by constructing a more sophisticated and delicate  gradient estimator. For example, SAG \citep{Nicolas2012}, SAGA \citep{Defazio2014} and SVRG  \citep{Johnson2013}, which yields  an overall   gradient complexity of $O(n^{3/2}\epsilon^{-1})$ \citep{Reddi2016b,Allen_Zhu2016}  to obtain an $\epsilon$-approximate first-order stationary point for nonconvex problems. These kind of variance reduction methods have  significant influence on the line of research, which is the first time that research  demonstrates that   stochastic gradient based methods   dominate deterministic gradient based methods in an order of $n^{1/3}$ for nonconvex optimization.
 
 However, we haven't touch the optimal result for nonconvex problems. Recently,  \cite{Fang2018} proposed a new variance reduction method named SPIDER, which achieves an overall $O(n^{1/2}\epsilon^{-1})$ gradient complexity to obtain an $\epsilon$-approximate first-order stationary point. This gradient complexity result is showed to be optimal when $n \le O(\epsilon^{-4})$.  
 
 
 However, the story is not over yet. There still exists an important issue under the structure of SPIDER. We first summarize the algorithm procedure of SPIDER below (only the inner loop of the algorithms is presented):
\begin{align}
	 v_k &= \sum_{i \in S} \nabla f_i(x_k) + \sum_{i \in S} \nabla f_i(x_{k-1}) + v_{k-1}, \label{spinder_old}\\
	 x_{k+1} &= x_k - \eta \frac{v_k}{\|v_k\|}. \label{NGD}
\end{align}
The procedure of SPIDER is different from the traditional SVRG, it uses a new gradient estimator (see \cref{spinder_old}), which uses $v_{k-1}$ instead of $v_0$ as compared to original SVRG methods. Furthermore, it uses a natural gradient descent  step instead of a gradient descent step in \cref{NGD}. The issue under this structure is that the convergence result can only be achieved under a strict condition that $\eta = O(\epsilon/L)$. This restriction is used to control the step length such that $\|x_{k+1} - x_k\| = O(\epsilon)$. Intuitively,  such a small movement makes it  possible to have a small variance for the gradient estimator.

 However, the requirement that step size $\eta$ is restrict to be smaller than the target accuracy $O(\epsilon)$  heavily hinders the practice application. Intuitively, if each step is restricted to be $O(\epsilon)$, it takes long time to arrive at a stationary point.  To overcome such issue, we learn form SPIDER and draw this variance reduction scheme back into the traditional SVRG. Our proposed SPIDER$^\textbf{+}$ algorithm is summarize as below:
\begin{align*}
v_k &= \sum_{i \in S} \nabla f_i(x_k) + \sum_{i \in S} \nabla f_i(x_{k-1}) + v_{k-1} \\
x_{k+1} &= x_k - \eta  {v_k} .  
\end{align*}
 We replace the NGD with normal gradient descent, which is more nature at the first glance. With a novel proof, the step size $\eta$ is bought back into life and can be as large as $O(1/L)$. The $\epsilon$ restriction is totally removed, which makes algorithm possible to live in  practical applications. In the meantime, the gradient complexity of  SPIDER$^\textbf{+}$ is the same as SPIDER. A detail comparison is summarized in \Cref{smooth_comparison}.

  
 \renewcommand{\arraystretch}{1.3} 
 \definecolor{LightCyan}{rgb}{0.88,1,1}
 \begin{table}[H] 
 	\small
 	\centering 
 	\begin{tabular}{clllll} \toprule
 		\multirow{2}{*}{Algorithms}& &\multirow{2}{*}{ $\eta$} &\multicolumn{1}{c}{Finite-Sum}   &\phantom{a}    &\multicolumn{1}{c}{Online} \\  
 		&& &\multicolumn{1}{c}{SFO}   & &\multicolumn{1}{c}{SFO}  \\   \midrule
 		GD &\citep{Nesterov2014}\footnotemark &$O( L^{-1} )$ &  $O(n \epsilon^{-1} )$  &  &- \\  \midrule
 		SGD &\citep{Ghadimi2016}\footnotemark &$O( L^{-1} )$  &  -   &  &$O(\epsilon^{-2}  )$    \\  \midrule 
 		
 		\multirow{2}{*}{SVRG}  &\citep{Reddi2016b}  &\multirow{2}{*}{$O( L^{-1}n^{-2/3} )$} & \multirow{2}{*}{$O( n^{2/3}\epsilon^{-1})$} &   &   \multirow{2}{*}{NA} \\ 
 		&\citep{Allen_Zhu2016}  \\ \midrule
 		
 		SCSG & \citep{Lei2017}  &$O( L^{-1}(n^{-2/3} \wedge \epsilon^{2/3} ))$ & $O(n^{2/3}\epsilon^{-1})$&   &   $O(  \epsilon^{-5/3}  )$  \\  \midrule
 		
 		SPIDER &\citep{Fang2018}\footnotemark   &$O( \epsilon L^{-1} )$ & $O(n^{1/2}\epsilon^{-1})$&   &   $O(  \epsilon^{-3/2}  )$  \\  \midrule \belowrulesepcolor{LightCyan}
 		\rowcolor{LightCyan}
 		SPIDER$^\textbf{+}$ &(This Work) &$O(L^{-1})$ & $O( n^{1/2}\epsilon^{-1})$&   &   $O(  \epsilon^{-3/2}  )$     \\   \aboverulesepcolor{LightCyan}  \bottomrule
 	\end{tabular} 
 	\vspace{2mm}
 	\caption{Comparable results on gradient complexity for smooth nonconvex  optimization. } \label{smooth_comparison}
 \end{table} 
 \footnotetext[1]{We note that for deterministic algorithms, the online setting does not exist.}  
  \footnotetext[2]{Actually, the SFO result of SGD in online setting is also applicable into finite-sum setting. However, divided it only into online setting makes the comparison more clear. }  
  \footnotetext[3] {Since SPIDER uses the natural gradient descent, if we seem it as GD, then the step size can be seem as $O(\epsilon L^{-1} /\|\nabla f(x_k)\|)$}.

 We compare the performance of algorithms in terms of stochastic frist-order oracle (SFO) and the step size $\eta$, where SFO is defined as given a point $x$ and a variable $\xi$, the SFO returns a stochastic gradient $\nabla f_\xi(x)$, and $\eta$ denotes the step size used in the descent step. Moreover, For the sake of clear comparison, we make a slightly different classification of finite-sum setting and online setting. The finite-sum setting and online setting correspond to the choices of $|S_1| = n$ and $ |S_1|  = O(\epsilon^{-a})$, respectively, where $|S_1|$ is the choice of batch size of outer loop in the algorithm, and $a$ is positive real number. If the algorithms do not have a clear outer loop and inner loop likes SVRG, we count $|S_1|$ as the batch size used in each iteration. We also note that the optimal result for an algorithm  can be achieved by a reasonable choosing of $|S_1| = \min \{n,  \epsilon^{-a}\}$, then the optimal SFO can be achieved as the minimum SFO between Finite-sum SFO and Online SFO. We refer readers to \cite{Lei2017,Li2018} for further exploration in this aspect. It is clear in \Cref{smooth_comparison} that the proposed SPIDER$^\textbf{+}$ achieves the best result among all algorithms in term of SFO in both finite-sum and online setting for smooth nonconvex optimization while still maintains a reasonable large step size $O(L^{-1})$, which is comparable to the step size used in GD.
  
Furthermore, with such a delicate algorithm in hand, we further extend it to nonsmooth nonconvex optimization and obtain an significant result. We consider a general constrained nonsmooth nonconvex finite-sum problem
 \begin{align*}
  \min_{x\in \mathcal{X}} 	\Psi(x)  \defeq  f(x)  + h(x),  \quad f(x) \defeq \frac{1}{n}\sum_{i=1}^{n} f_i(x),  \tag{P2}
 \end{align*}
where $\mathcal{X}$ is a closed convex set in Euclidean space $\mathbb{R}^d$, $f: \mathcal{X} \rightarrow \mathbb{R} $ is the average of $n$ continuously differentiable functions $f_i: \mathcal{X} \rightarrow \mathbb{R} $, but possibly nonconvex, and $h: \mathcal{X} \rightarrow \mathbb{R} $ is simple convex function, but possibly nonsmooth.  If $h(x) \equiv 0$ and $\mathcal{X} = \mathbb{R}^d$, then this problem reduces to a simple smooth nonconvex problem. However, in many machine learning problems, $h(x)$ is often a nonsmooth  regularizer such that the obtained minimizer $x^\star$ has specific structure. For example, $h(x) = \|x\|_1$  induces sparsity for the obtained minimizer.  We proposed a proximal SPIDER$^\textbf{+}$ algorithm (ProxSPIDER$^\textbf{+}$) and achieves the total gradient complexity of $n^{1/2}\epsilon^{-1}$ to obtain an $\epsilon$-approximate solution, which is the best result in proximal first-order algorithm to the best of our knowledge. We summarize our result in \Cref{comparison_nonsmooth}. For nonsmooth nonconvex optimization, we introduction another oracle the proximal oracle (PO), which is defined as given a point $x$ and the gradient estimator $v$, PO returns the solution of the proximal projection. As shown in \Cref{comparison_nonsmooth} our result improves the previous result by an order of $O(n^{1/6})$ in terms of SFO on finite-sum setting.


Furthermore,  we also consider SPIDER$^\textbf{+}$ and ProxSPIDER$^\textbf{+}$ under \emph{online optimization} setting, where the sample size $n$ is too large or even infinite. Then, taking a full batch samples at each outer loop is not efficient or even impossible. In fact, to obtain an $\epsilon$ accuracy, the full batch is not necessary. By taking sample size of the outer loop  in the order of $O(\epsilon^{-1/2})$, we show that the total gradient complexity is $O(\epsilon^{-3/2})$ for both \emph{smooth} (P1) and \emph{nonsmooth} (P2) problems to achieve the $\epsilon$ accuracy. Especially, to the best of our knowledge, our result  $O(\epsilon^{-3/2})$ on nonsmooth problem is new in literature,  and is the best result in proximal first-order method, which improves the SFO in the previous study in an order of $\epsilon^{1/6}$ on online setting.

\textbf{Notation}  For a vector $x$, $\|x\|$ denotes the $\ell_2$ norm of the vector $ x$.   We use $\nabla f(\cdot)$   to denote  gradient of $f(\cdot)$. $\mathbb{R}$, $\mathbb{R}^+$ and $\mathbb{R}^d$ denote the set of all real numbers,  non-negative real numbers and $d$-dimension real vectors, respectively.  
 


==> introduction_oldv2.tex <==
\vspace{-7mm}
\section{Introduction}

Large-scale machine learning problems can often be formulated as the following finite-sum optimization problem
\begin{align}
\min_{x\in \mathbb{R}^d}	\Psi(x)  \defeq f(x) , ~\text{where}~ f(x) \defeq \frac{1}{n}\sum_{i=1}^{n} f_i(x)  \tag{P}
\end{align}
where the function $f$ denotes the total loss on the training samples and in general is nonconvex. Since the sample size $n$ can be very large, the full-batch gradient descent algorithm has high computational complexity. Various stochastic gradient descent (SGD) algorithms have been proposed and extensively studied. For nonconvex optimization, the basic SGD algorithm, which calculates one gradient per iteration, has been shown to yield an overall stochastic first-order oracle (SFO) complexity, i.e., gradient complexity, of $\mathcal{O}(\epsilon^{-4})$ \citep{Ghadimi2013} to attain a first-order stationary point $\bar{x}$ that satisfies $\mathbb{E}\|\nabla f(\bar{x})\|  \le \epsilon$. SGD algorithms with diminishing  step-size \citep{Bottou2018} or a sufficiently large batch size \citep{Ghadimi2016,ZhouHybird2018} were further proposed to guarantee their convergence to a stationary point rather than its neighborhood.
 
Furthermore, various variance reduction methods have been proposed by constructing more accurate gradient estimators such as SAG \citep{Nicolas2012}, SAGA \citep{Defazio2014} and SVRG \citep{Johnson2013}. In particular, SAGA and SVRG have been shown to yield  an overall SFO complexity of $O(n^{2/3}\epsilon^{-2})$ \citep{Reddi2016b,Allen_Zhu2016}.
%, which  dominates deterministic gradient descent methods with an order of $\mathcal{O}(n^{1/3})$ for nonconvex optimization.
 Recently, \citep{Lam2017a,Lam2017b} proposed a novel variance reduction method SARAH, where the gradient estimator is sequentially updated in the inner loop to improve the estimation accuracy. In particular, SARAH 
%takes the stepsize $\eta=\mathcal{O}(1/(L\sqrt{q}))$ (where $q$ is the number of iterations in each inner loop), and 
has been shown in \citep{Lam2017b} to achieve an overall $\mathcal{O}(\epsilon^{-4})$ SFO complexity for nonconvex optimization. Another  method SPIDER of the same type was   proposed in \citep{Fang2018}, which uses the same gradient estimator as SARAH but adopts a natural gradient update with a stepsize $\eta=\mathcal{O}(\epsilon/L)$.\footnote{SPIDER 
%in \citep{Fang2018} takes a natural gradient descent with a stepsize $\eta=\mathcal{O}(\epsilon/L)$. It 
can also be viewed as a gradient descent update with an adaptive stepsize $\eta_k=\mathcal{O}(\epsilon/\left(L\|v_k\|\right))$, where $ \|v_k\|\geq \epsilon$ is the estimate of the gradient at the $k$-th step. During the initial stage of the algorithm, $ \|v_k\|$ can be much larger than $\epsilon$ so that the resulting stepsize can be very small.} \citep{Fang2018} showed that SPIDER achieves an overall $\mathcal{O}(\min\{ n^{1/2}\epsilon^{-2}, \epsilon^{-3 }\})$ SFO, which was further shown to be optimal in the regime $n \le \mathcal{O}(\epsilon^{-4})$. 

Though SPIDER is theoretically appealing, three important issues still require further attention. First, SPIDER requires a very restrictive stepsize $\eta=\mathcal{O}(\epsilon/L)$ to guarantee its convergence, which prevents SPIDER from making big progress even if it is possible. Relaxing such a condition appears not easy under its original convergence analysis framework. 
%Thus, the first question we ask is:
\begin{list}{$\bullet$}{\topsep=0.ex \leftmargin=0.15in \rightmargin=0.in \itemsep =-0.05in}
%\item {\em Can we  relax the parameter restrictions of SPIDER without losing the guaranteed convergence rate? }
\item {\em In this paper, we propose the SpiderBoost algorithm, which allows a much larger stepsize $\eta =\mathcal{O}(1/L)$ than SPIDER 
%$\eta =\mathcal{O}(\epsilon/\left(L\|v_k\|\right))$ adopted by SPIDER (if viewed under the gradient descent update), 
while retaining the same state-of-the-art complexity order as SPIDER (see \Cref{smooth_comparison} in Suppl). This is due to the new convergence analysis idea that we develop, which analyzes the increments of variables over each entire inner loop  rather than over each inner-loop iteration, and hence yields tighter bound and consequently more relaxed stepsize requirement. The advantage of SpiderBoost over SPIDER is further demonstrated via experiments.
%As a result, SpiderBoost achieves significantly larger progress towards a first-order stationary point than SPIDER especially in the initial optimization phase where $\|v_k\|$ is large, as demonstrated in \Cref{Experment_1}.  
}
\end{list}

Second, the convergence analysis of SPIDER requires a very small per-iteration increment $\|x_{k+1}-x_k\|=\mathcal{O}(\epsilon/L)$, which is difficult to guarantee if one attempts to generalize it to a proximal algorithm for solving a composite optimization problem, due to the nonlinearity of the proximal operator. Hence, generalizing SPIDER to proximal algorithms with provable convergence guarantee is challenging.
%, if not impossible. Thus, the second question we ask is:
\begin{list}{$\bullet$}{\topsep=0.ex \leftmargin=0.15in \rightmargin=0.in \itemsep =-0.05in}
%\item {\em If an improved SPIDER can be designed, does such improvement facilitates the generalization to proximal algorithms with convergence guarantee? Does the resulting algorithm improves the SFO complexity of existing proximal algorithms?}
\item {\em
\end{list}

Third, although SPIDER achieves the optimal stochastic gradient oracle complexity in nonconvex optimization, its practical performance has been found in recent works \cite{Lam2017b,Fang2018} to be hardly advantageous to that of the traditional SVRG. Therefore, it is of vital importance to exploit other algorithmic dimensions to further improve the practical performance of SPIDER. Momentum is such a promising perspective. However, there are still two major challenges ahead to design momentum schemes for variance-reduced algorithms in nonconvex optimization. First, while momentum scheme has been well studied for (stochastic) gradient algorithms \cite{Ghadimi2016prox} in nonconvex optimization, the convergence guarantee of stochastic variance-reduced-like algorithms is only explored for SVRG in certain convex scenarios \cite{Nitanda2016,Allen-Zhu2017,Allen-Zhu2018,Shang2018}. Therefore, it is not even clear whether a certain momentum scheme can be applied to stochastic variance-reduced algorithms based on SPIDER and yield the optimal oracle gradient complexity for nonconvex optimization. Furthermore, the existing momentum scheme for stochastic algorithms to solve the composite nonconvex problem has convergence guarantee only for convex regularizers $g$ that have a bounded domain \cite{Ghadimi2016prox}, which are not applicable to a variety of application scenarios where regularizers with unbounded domain (e.g., $\ell_1, \ell_2$) are commonly used. Thus, the third question we ask is:
\begin{list}{$\bullet$}{\topsep=0.ex \leftmargin=0.15in \rightmargin=0.in \itemsep =-0.05in}
\item {\em Can we design a SPIDER type of algorithm with momentum, which has an optimal oracle gradient complexity for nonconvex optimization, and allows a much broader choice of regularizers than the existing algorithm?}
\end{list}


Our study provides affirmative answers to these questions. 
%Our contributions are summarized as follows.



%%%%%%%%

%In this paper, we study  the following nonconvex and nonsmooth composite optimization problem
%\begin{align}\label{objecP}
%\min_{x\in \mathbb{R}^d} \Psi(x):=f(x)+h(x), \tag{P}
%\end{align}
%where $h(x)$ is a simple but nonsmooth convex function and $f(x)$ has the following finite-sum form 
%\begin{align}
%f(x)=\frac{1}{n}\sum_{i=1}^n f_i(x),
%\end{align}
%where $l_i(x), i=1,...,n$ are $n$ individual nonconvex and smooth functions. 
% Such a problem has attracted a lot attention in many regularized machine learning problems, e.g., egularized empirical risk minimization problems~\cite{??}.  To handle the non-smoothness  of the function $h(x)$, one natural way is to conduct the following proximal update 
%\begin{align}
%x_{k+1} = \mathrm{prox}_{\eta h}(x_k - \eta v_k)
%\end{align}
%at the $k^{th}$ iteration, where the proximal mapping is given by 
%\begin{align}\label{pmap}
%	\text{(Proximal mapping):}~\mathrm{prox}_{\eta h}(x):= \arg\min_{u\in\mathbb{R}^d} \Big\{h(u) + \frac{1}{2\eta}\|u-x\|^2\Big\}.  
%\end{align}
%and $v_k$ is the stochastic gradient estimation of $\nabla f(x_k)$. Based on such a technique,  \cite{Ghadimi2016} proposed a proximal stochastic gradient decent (ProxSGD) by picking $v_k=\nabla \ell_{i_k}f(x_k)$ with $i_{k}$ chosen from $\{1,...,n\}$ uniformly at random, and proposed a proximal gradient decent (ProxGD) by choosing $v_k=\nabla f(x_k)$. Measured by the stochastic first-order (SFO) complexity that is the number of computation of stochastic gradients,  and the proximal oracle (PO) complexity that is the number of computation of proximal projections,  ProxSGD and ProxGD achieve a SFO complexity of $\mathcal{O}(\min\{n\epsilon^{-1}, \epsilon^{-2}\})$ and a PO complexity of $\mathcal{O}(\epsilon^{-1})$ to obtain a $\epsilon$-approximate first-order stationary point, i.e., $\mathbb{E}\|\nabla G_{\eta}(x)\|^2\leq \epsilon$, where $G_{\eta}(x)$ is the generalized gradient of function $\Psi(\cdot)$ at the point $x$. To accelerate the convergence rate, the stochastic variance reduced gradient (SVRG) based and the SAGA based proximal algorithms were proposed by \cite{Reddi2016,Allen_Zhu2017,Li2018} and achieved a SFO complexity of $\mathcal{O}(\min\{n^{2/3}\epsilon^{-1},\epsilon^{-5/3}\})$,  which improve the SFO complexity of ProxSGD and ProxGD by a factor of $\mathcal{O}(\min\{n^{1/3},\epsilon^{-1/3}\})$.  
%
% Recently,  \cite{Fang2018} proposed a new variance reduction technique named Spider for solving the finite-sum nonconvex optimization problem, i.e., the problem~\eqref{objecP} with $h(x)\equiv0$, which achieves a near-optimal gradient complexity to obtain an $\epsilon$-approximate first-order stationary point. Thus, one natural question is 
% \begin{align*}
% \textit{Can we further improve the SFO complexity of existing proximal algorithms by Spider?} 
%\end{align*}
%We answer this question affirmably  but by using a more practical variant of Spider, which we call as SpiderBoost. Compared with Spider, our developed SpiderBoost has two main advantages. First, SpiderBoost allows a much larger stepsize $\eta_k=\mathcal{O}(1/L)$ than the stepsize $\eta_k=\mathcal{O}(\epsilon/\left(L\|v_k\|\right)), \|v_k\|\geq \epsilon$ adopted by Spider without any theoretical performance loss. As a result, our SpiderBoost achieves significantly larger progress towards to the first-order stationary point than Spider especially in the initial optimization phase where $\|v_k\|$ is large, as demonstrated in our experiment.  Second, Spider  requires a extremely small per-iteration increment $\|x_{k+1}-x_k\|=\mathcal{O}(\epsilon/L)$, whereas  our SpiderBoost only needs $\|x_{k+1}-x_k\|$ to be $\mathcal{O}(1/L)$. Such a flexibility makes our SpiderBoost more easily extend to the proximal algorithm than Spider, as restricting the proximal projection within a $\mathcal{O}(\epsilon)$ region is challenging both in the theoretical analysis and the practical usage. % large increment  $\|x_{k+1}-x_k\|=\mathcal{O}(1/L)$, whereas SPIDER requires $x_{k+1}-x_{k}=\mathcal{O}(\epsilon/L)$.
%%$\ell_i(\cdot): \mathbb{R}^d \rightarrow \mathbb{R}$ corresponds to the loss function on the $i$-th data sample and function $h$ denotes the regularizer that promotes desired structures to the solution based on our prior knowledge. Due to the big data trend, the demanding large data size $n$ makes it impossible to apply gradient descent method, which hiders the  efficiency of gradient descent (GD) and leads to  an overall gradient complexity of $O( n\epsilon^{-1})$ \citep{Nesterov2014} to obtain an $\epsilon$-approximate first-order stationary point. On the other hand, SGD is a possible candidate algorithm due to its low per-iteration sample complexity. However, its applicability is restricted by its notoriously slow convergence rate.
\subsection{Summary of Contributions}


\renewcommand{\arraystretch}{0.6} 
\definecolor{LightCyan}{rgb}{0.88,1,1}


\begin{table*}[t] 
	\small
	\centering 
	\caption{Comparison of results on SFO compelxity and PO compelxity for nonconvex and nonsmooth optimization.} \label{comparison_nonsmooth}
	\vspace{2mm}
\scalebox{0.9}{	
	\begin{threeparttable} 
			\begin{tabular}{clllcll} \toprule
				\multirow{2}{*}{Algorithms}& &\multirow{2}{*}{Stepsize $\eta$} &\multicolumn{2}{c}{Finite-Sum}       &\multicolumn{2}{c}{Finite-Sum/Online} \\ 
				\cmidrule{4-5}   \cmidrule{6-7} 
				&  & &\multicolumn{1}{c}{SFO\footnotemark} &\multicolumn{1}{c}{PO}    &\multicolumn{1}{c}{SFO} &\multicolumn{1}{c}{PO} \\   \midrule
				%		ProxGD &\citep{Ghadimi2016}\footnotemark &$\mathcal{O}(L^{-1})$ &  $\mathcal{O}(n \epsilon^{-1} )$    & $\mathcal{O}( \epsilon^{-1} )$   & & \\ \midrule
				
				ProxGD  &\citep{Ghadimi2016} &$\mathcal{O}(L^{-1})$  & $\mathcal{O}(n \epsilon^{-2} )$   &  $\mathcal{O}( \epsilon^{-2} )$ &N/A  &N/A \\ \midrule
				
				ProxSGD &\citep{Ghadimi2016} &$\mathcal{O}(L^{-1})$  & N/A   &  N/A &$\mathcal{O}(\epsilon^{-4}  )$   &$\mathcal{O}( \epsilon^{-2} )$ \\ \midrule
				
				
				ProxSVRG/SAGA &\citep{Reddi2016} &$\mathcal{O}(L^{-1})$ &  $\mathcal{O}(n+ n^{2/3} \epsilon^{-2}  )$    & $\mathcal{O}( \epsilon^{-2} )$  &N/A &N/A \\ \midrule
				
				Natasha1.5  &\citep{Allen_Zhu2017} &$\mathcal{O}(\epsilon^{2/3}L^{-2/3})$ &N/A &N/A    &  $\mathcal{O}(\epsilon^{-3}+  \epsilon^{-10/3}   )$    & $\mathcal{O}( \epsilon^{-10/3} )$  \\ \midrule
				
				ProxSVRG$^\textbf{+}$ &\citep{Li2018} \footnotemark &$\mathcal{O}(L^{-1})$&$\mathcal{O}(n^{2/3}\epsilon^{-2})$& $\mathcal{O}(\epsilon^{-2})$ &   $\mathcal{O}(  \epsilon^{-10/3}  )$    & $\mathcal{O}( \epsilon^{-2} )$   \\  \midrule
				
				\belowrulesepcolor{LightCyan}   
				\rowcolor{LightCyan}
				Prox-SpiderBoost &(This Work) &$\mathcal{O}(L^{-1})$ & $\mathcal{O}(n+ n^{1/2}\epsilon^{-2})$&  $\mathcal{O}(\epsilon^{-2})$ &    $\mathcal{O}(  \epsilon^{-2} + \epsilon^{-3 }  )$    & $\mathcal{O}( \epsilon^{-2} )$  \\   \aboverulesepcolor{LightCyan}  \bottomrule
		\end{tabular}  	 
		\vspace{2mm}
		\begin{tablenotes}\small
			\item[5] For a fair comparison, we note that \cite{Li2018} make an additional assumption that the total number of iterations is a multiple of the number of inner loop iterations. Under such assumption, ProxSVRG/ProxSAGA \cite{Reddi2016} and Prox-SpiderBoost (this work) have SFO given by $n^{2/3}\epsilon^{-2}$ and $n^{1/2}\epsilon^{-2}$, respectively.
			\item[6]  {\citep{Li2018} contains a detailed discussion on the choice of the outer-loop batch size. Here, we include only their best result.} 
		\end{tablenotes}
	\end{threeparttable} 
}
\end{table*} 
 
Inspired by SARAH and SPIDER, we propose a more practical variant named SpiderBoost. 
%SpiderBoost has two main advantages. (1) 
SpiderBoost allows a much larger stepsize $\eta =\mathcal{O}(1/L)$ than $\eta =\mathcal{O}(\epsilon/\left(L\|v_k\|\right))$ adopted by SPIDER (if viewed under the gradient descent update), and at the same time achieves the same state-of-the-art complexity order as SPIDER (see \Cref{smooth_comparison}). This is due to the new convergence analysis idea that we develop, which analyzes the increments of variables over each entire inner loop  rather than over each inner-loop iteration, and hence yields tighter bound and consequently more relaxed stepsize requirement. As a result, SpiderBoost achieves significantly larger progress towards a first-order stationary point than SPIDER especially in the initial optimization phase where $\|v_k\|$ is large, as demonstrated in \Cref{Experment_1}.  

SpiderBoost comes with a natural generalization, i.e., the Prox-SpiderBoost algorithm, which we propose for solving the composite problem (Q) (see \Cref{sec_proximal}), where the objective function consists of a finite-sum nonconvex function and a convex but nonsmooth regularizer function. Since the convergence analysis we develop for SpiderBoost does not require a bound on $\|x_{k+1}-x_k\|$ as in SPIDER, it significantly facilitates the convergence analysis for proximal algorithms. In particular, we show that Prox-SpiderBoost achieves a  SFO  complexity of $\mathcal{O}( n^{1/2}\epsilon^{-2} )$ and a proximal oracle (PO)  complexity of $\mathcal{O}(\epsilon^{-2})$. Such a SFO complexity improves the existing best results by a factor of $\mathcal{O}( n^{1/6} )$ (see \Cref{comparison_nonsmooth}). 

%, which is in contrast to SPIDER, which explicitly exploits the condition $\|x_{k+1}-x_k\|=\mathcal{O}(\epsilon/L)$ and has difficulty to hold for proximal algorithms.


%%Such a flexibility significantly facilitates SpiderBoost to be extended to proximal algorithms for solving composite optimization, whereas SPIDER does not come with such an attribute, because restricting the proximal projection within a $\mathcal{O}(\epsilon)$ region is challenging both in the theoretical analysis and the practical usage. % large increment  $\|x_{k+1}-x_k\|=\mathcal{O}(1/L)$, whereas SPIDER requires $x_{k+1}-x_{k}=\mathcal{O}(\epsilon/L)$.
%%%$\ell_i(\cdot): \mathbb{R}^d \rightarrow \mathbb{R}$ corresponds to the loss function on the $i$-th data sample and function $h$ denotes the regularizer that promotes desired structures to the solution based on our prior knowledge. Due to the big data trend, the demanding large data size $n$ makes it impossible to apply gradient descent method, which hiders the  efficiency of gradient descent (GD) and leads to  an overall gradient complexity of $O( n\epsilon^{-1})$ \citep{Nesterov2014} to obtain an $\epsilon$-approximate first-order stationary point. On the other hand, SGD is a possible candidate algorithm due to its low per-iteration sample complexity. However, its applicability is restricted by its notoriously slow convergence rate.
%
%Taking the aforementioned second advantage, we propose Prox-SpiderBoost for solving the composite problem (Q) (see \Cref{sec_proximal}), where the objective function consists of a finite-sum nonconvex function and a convex but nonsmooth   regulizer function. We show that Prox-SpiderBoost achieves a  SFO  complexity of $\mathcal{O}( n^{1/2}\epsilon^{-2} )$ and a proximal oracle (PO)  complexity of $\mathcal{O}(\epsilon^{-2})$. Such a SFO complexity improves the existing best results by a factor of $\mathcal{O}( n^{1/6} )$ (see \Cref{comparison_nonsmooth}). We further extend Prox-SpiderBoost  for solving the constrained composite optimization problem using the proximal mapping under a non-Euclidean geometry. Under certain conditions, we prove that the obtained algorithm achieves the same SFO complexity and PO complexity as Prox-SpiderBoost for solving the unconstrained problem~(Q). For nonconvex composite optimization problems that satisfy the so-called $\tau$-Polyak-{\L}ojasiewicz condition (see \Cref{def: sc}), we propose a variant of the Prox-SpiderBoost algorithm and establish its oracle complexity result for finding a stationary point. Our proposed algorithm achieves a SFO complexity of $\mathcal{O}((n+\tau^2)\log ({1}/{\epsilon}))$, which outperforms the existing state-of-art complexity bounds  in several regions (see \Cref{comparison_nonsmooth_gd}).
%
%We finally propose and study Prox-SpiderBoost-O  for online stochastic composite optimization, where the objective function takes the form $f(x)=\mathbb{E}_{\zeta} [f_{\zeta}(x)]$ with the expectation over the underlying data distribution rather than the finite-sum form. Our results show that Prox-SpiderBoost-O achieves a SFO complexity of $\mathcal{O}(\epsilon^{-3 })$ for nonconvex optimizations, which improves the existing best SFO complexity $\mathcal{O} (\epsilon^{-10/3})$ (see \Cref{comparison_nonsmooth})  by a factor of $\mathcal{O}(\epsilon^{-1/3})$. The same complexity result also holds for the general constrained optimization under a non-Euclidean geometry. 

Based on Spiderboost, we further propose Proximal SPIDER-M, which is a proximal stochastic algorithm that exploits both the SPIDER variance-reduction scheme and a momentum scheme for solving the composite problem (Q). We show that the output point generated by the Proximal SPIDER-M satisfies a generalized $\epsilon$-first-order stationary condition within $O(\epsilon^{-2})$ number of iterations, and the corresponding stochastic gradient oracle complexity is in the order of $O(n+\sqrt{n} \epsilon^{-2})$, matching the complexity lower bound for nonconvex optimization. To the best of our knowledge, this is the first known theoretical guarantee for stochastic variance-reduced type of algorithms with momentum in nonconvex optimization. We also note that the design of our momentum scheme is applicable to arbitrary convex regularizers, which significantly relaxes the constraint of the existing momentum scheme that requires the regularizer to have a bounded domain in order to have a convergence guarantee for nonconvex optimization \cite{Ghadimi2016prox}.

Due to the space limitations, we relegate our results on several topics to the supplementary materials including Prox-SpiderBoost for solving constrained composite optimization under a non-Euclidean geometry, unconstrained composite optimization under the $\tau$-Polyak-{\L}ojasiewicz condition, and online stochastic composite optimization, and Proximal SPIDER-M for online nonconvex composite optimization.

\subsection{Related Work}

Due to a significant amount of studies on stochastic first-order algorithms, we here include only the highly relevant work to our results.

{\bf SGD for smooth nonconvex optimization:} 
%Stochastic first-order algorithms for smooth nonconvex optimization have been well studied. 
The convergence analysis for SGD was studied in \citep{Ghadimi2013} for smooth nonconvex optimization. SGD with diminishing stepsize and sufficiently large batch size were further studied in \citep{Ghadimi2016,Bottou2018,ZhouHybird2018} to improve the performance. 
 
 {\bf Variance reduced algorithms for smooth nonconvex optimization:} Various variance-reduced algorithms have been proposed and studied to improve the performance of SGD type of algorithms for smooth nonconvex optimization, including , e.g., SVRG \citep{Johnson2013,Reddi2016b,Allen_Zhu2016}, SCSG \citep{Lei2017}, and SNVRG \citep{Zhou2018}.

New variance reduction algorithms SARAH \cite{Lam2017a,Lam2017b} and SPIDER \cite{Fang2018} have been proposed for smooth nonconvex optimization, which recursively update the gradient estimator based on fresh samples at each inner-loop iteration to further improve the performance. In particular, SPIDER has been shown in \citep{Fang2018} to be optimal for a certain regime. Such an idea has also been extended for optimization over manifolds in \citep{ZhouPan2018,Zhang2018}. Our study here proposes a SpiderBoost algorithm, which substantially improves the stepsize of SPIDER under the same performance guarantee and performs much faster than SPIDER in practice.
%Although SPIDER was shown to be near-optimal in certain regime, the strict restriction of stepsize makes SPIDER type algorithms converge slowly in practice. We propose a new algorithm scheme named SpiderBoost to overcome the small stepszie restriction, and hence boosts  SPIDER both in theory and practice.
 
{\bf Stochastic algorithms for nonsmooth nonconvex optimization:} Proximal SGD has been proposed and studied by \citep{Ghadimi2016,Ghadimi2016prox} to solve nonsmooth nonconvex optimization problems. Moreover, variance reduced algorithms such as Prox-SVRG and Prox-SAGA \cite{Reddi2016}, Natasha1.5 \cite{Allen_Zhu2017}, and ProxSVRG$^+$ \cite{Li2018} have also been proposed to further improve the performance. Our study here first improves the design of SPIDER, and then leverages such advantage and  proposes Prox-SpiderBoost, which we show order-level outperforms all the existing algorithms for nonsmooth nonconvex optimization. 

\textbf{Momentum schemes for nonconvex optimization:}
Momentum scheme is originally designed for accelerating gradient algorithms to achieve an optimal convergence rate in convex optimization \cite{Nesterov2014,Beck2009,Tseng2010,Ghadimi2016prox}. For nonconvex optimization, \cite{Ghadimi2016prox} established convergence of stochastic gradient algorithms with momentum to an $\epsilon$-first-order stationary point with an overall stochastic gradient oracle complexity of $O(\epsilon^{-4})$. 
The convergence guarantee of SVRG with momentum has been explored under a certain local gradient dominance geometry in nonconvex optimization \cite{Li2017}. However, the momentum scheme there requires to compare the objective function value (and hence calculate the total loss) at each iteration and hence is not sample efficient. Similar momentum scheme has also been explored in second-order algorithms for nonconvex optimization \cite{Wang2018}.


%{\bf SARAH and SPIDER for nonsmooth nonconvex optimization:} 
% Due to the strict restriction of stepszie, simple generalization of SPIDER to nonsmooth nonconvex optimization fails. However, SpiderBoost does not have such issue. We propose a generalization version of SpiderBoost named Prox-SpiderBoost, which outperforms all the existing algorithms in order level! Prox-SpiderBoost is also the first SARAH and SPIDER type algorithm that has capability to handle nonsmooth nonconvex optimization.

\noindent\textbf{Notations:}  For a vector $x \in \mathbb{R}^d$, $\|x\|$ denotes its $\ell_2$ norm.   We use $\nabla f$   to denote the gradient of $f$. We use $\mathbb{R}$, $\mathbb{R}^+$ and $\mathbb{R}^d$ to denote the set of all real numbers,  non-negative real numbers, and $d$-dimension real vectors, respectively.  


%------------------------------------------------------------------------------------ (zhe "s )

% To overcome such issue and reduce the dependent on $n$, stochastic gradient descent method  (SGD) is proposed, which calculates one gradient per iteration and yields an overall gradient complexity of $O(\epsilon^{-2})$ \citep{Ghadimi2016}, which is also its convergence rate since it only calculates one gradient per iteration. SGD efficiently drops the dependent on $n$, but the convergence rate is slower as compared to $O(\epsilon^{-1})$ convergence rate of GD and is more rely on the target accuracy $\epsilon$. Moreover, the vanilla SGD can only converge to the neighbor of first-order stationary points instead of the exact stationary points. The inexact convergence issue can be eliminated by diminishing the step-size \citep{Bottou2018} or choose a sufficient large batch size in each iteration.  
% 
% However, the slow convergence issue still hiders the application of stochastic gradient-based method in various situation, especially for   machine learning problems that requires high accuracy solutions. Fortunately, this issue has been identified as variance issue, which caused by the inexact estimation of using stochastic gradient to estimate the full gradient. Thus, various variance reduction methods have been proposed to reduce the variance of the gradient estimator  by constructing a more sophisticated and delicate  gradient estimator. For example, SAG \citep{Nicolas2012}, SAGA \citep{Defazio2014} and SVRG  \citep{Johnson2013}, which yields  an overall   gradient complexity of $O(n^{3/2}\epsilon^{-1})$ \citep{Reddi2016b,Allen_Zhu2016}  to obtain an $\epsilon$-approximate first-order stationary point for nonconvex problems. These kind of variance reduction methods have  significant influence on the line of research, which is the first time that research  demonstrates that   stochastic gradient based methods   dominate deterministic gradient based methods in an order of $n^{1/3}$ for nonconvex optimization.
% 
% However, we haven't touch the optimal result for nonconvex problems. Recently,  \cite{Fang2018} proposed a new variance reduction method named SPIDER, which achieves an overall $O(n^{1/2}\epsilon^{-1})$ gradient complexity to obtain an $\epsilon$-approximate first-order stationary point. This gradient complexity result is showed to be optimal when $n \le O(\epsilon^{-4})$.  
% 
% 
% However, the story is not over yet. There still exists an important issue under the structure of SPIDER. We first summarize the algorithm procedure of SPIDER below (only the inner loop of the algorithms is presented):
%\begin{align}
%	 v_k &= \sum_{i \in S} \nabla f_i(x_k) + \sum_{i \in S} \nabla f_i(x_{k-1}) + v_{k-1}, \label{spinder_old}\\
%	 x_{k+1} &= x_k - \eta \frac{v_k}{\|v_k\|}. \label{NGD}
%\end{align}
%The procedure of SPIDER is different from the traditional SVRG, it uses a new gradient estimator (see \cref{spinder_old}), which uses $v_{k-1}$ instead of $v_0$ as compared to original SVRG methods. Furthermore, it uses a natural gradient descent  step instead of a gradient descent step in \cref{NGD}. The issue under this structure is that the convergence result can only be achieved under a strict condition that $\eta = O(\epsilon/L)$. This restriction is used to control the step length such that $\|x_{k+1} - x_k\| = O(\epsilon)$. Intuitively,  such a small movement makes it  possible to have a small variance for the gradient estimator.
%
% However, the requirement that step size $\eta$ is restrict to be smaller than the target accuracy $O(\epsilon)$  heavily hinders the practice application. Intuitively, if each step is restricted to be $O(\epsilon)$, it takes long time to arrive at a stationary point.  To overcome such issue, we learn form SPIDER and draw this variance reduction scheme back into the traditional SVRG. Our proposed SPIDER$^\textbf{+}$ algorithm is summarize as below:
%\begin{align*}
%v_k &= \sum_{i \in S} \nabla f_i(x_k) + \sum_{i \in S} \nabla f_i(x_{k-1}) + v_{k-1} \\
%x_{k+1} &= x_k - \eta  {v_k} .  
%\end{align*}
% We replace the NGD with normal gradient descent, which is more nature at the first glance. With a novel proof, the step size $\eta$ is bought back into life and can be as large as $O(1/L)$. The $\epsilon$ restriction is totally removed, which makes algorithm possible to live in  practical applications. In the meantime, the gradient complexity of  SPIDER$^\textbf{+}$ is the same as SPIDER. A detail comparison is summarized in \Cref{smooth_comparison}.
%
%  
% \renewcommand{\arraystretch}{1.3} 
% \definecolor{LightCyan}{rgb}{0.88,1,1}
% \begin{table}[H] 
% 	\small
% 	\centering 
% 	\begin{tabular}{clllll} \toprule
% 		\multirow{2}{*}{Algorithms}& &\multirow{2}{*}{ $\eta$} &\multicolumn{1}{c}{Finite-Sum}   &\phantom{a}    &\multicolumn{1}{c}{Online} \\  
% 		&& &\multicolumn{1}{c}{SFO}   & &\multicolumn{1}{c}{SFO}  \\   \midrule
% 		GD &\citep{Nesterov2014}\footnotemark &$O( L^{-1} )$ &  $O(n \epsilon^{-1} )$  &  &- \\  \midrule
% 		SGD &\citep{Ghadimi2016}\footnotemark &$O( L^{-1} )$  &  -   &  &$O(\epsilon^{-2}  )$    \\  \midrule 
% 		
% 		\multirow{2}{*}{SVRG}  &\citep{Reddi2016b}  &\multirow{2}{*}{$O( L^{-1}n^{-2/3} )$} & \multirow{2}{*}{$O( n^{2/3}\epsilon^{-1})$} &   &   \multirow{2}{*}{NA} \\ 
% 		&\citep{Allen_Zhu2016}  \\ \midrule
% 		
% 		SCSG & \citep{Lei2017}  &$O( L^{-1}(n^{-2/3} \wedge \epsilon^{2/3} ))$ & $O(n^{2/3}\epsilon^{-1})$&   &   $O(  \epsilon^{-5/3}  )$  \\  \midrule
% 		
% 		SPIDER &\citep{Fang2018}\footnotemark   &$O( \epsilon L^{-1} )$ & $O(n^{1/2}\epsilon^{-1})$&   &   $O(  \epsilon^{-3/2}  )$  \\  \midrule \belowrulesepcolor{LightCyan}
% 		\rowcolor{LightCyan}
% 		SPIDER$^\textbf{+}$ &(This Work) &$O(L^{-1})$ & $O( n^{1/2}\epsilon^{-1})$&   &   $O(  \epsilon^{-3/2}  )$     \\   \aboverulesepcolor{LightCyan}  \bottomrule
% 	\end{tabular} 
% 	\vspace{2mm}
% 	\caption{Comparable results on gradient complexity for smooth nonconvex  optimization. } \label{smooth_comparison}
% \end{table} 
% \footnotetext[1]{We note that for deterministic algorithms, the online setting does not exist.}  
%  \footnotetext[2]{Actually, the SFO result of SGD in online setting is also applicable into finite-sum setting. However, divided it only into online setting makes the comparison more clear. }  
%  \footnotetext[3] {Since SPIDER uses the natural gradient descent, if we seem it as GD, then the step size can be seem as $O(\epsilon L^{-1} /\|\nabla f(x_k)\|)$}.
%
% We compare the performance of algorithms in terms of stochastic frist-order oracle (SFO) and the step size $\eta$, where SFO is defined as given a point $x$ and a variable $\xi$, the SFO returns a stochastic gradient $\nabla f_\xi(x)$, and $\eta$ denotes the step size used in the descent step. Moreover, For the sake of clear comparison, we make a slightly different classification of finite-sum setting and online setting. The finite-sum setting and online setting correspond to the choices of $|S_1| = n$ and $ |S_1|  = O(\epsilon^{-a})$, respectively, where $|S_1|$ is the choice of batch size of outer loop in the algorithm, and $a$ is positive real number. If the algorithms do not have a clear outer loop and inner loop likes SVRG, we count $|S_1|$ as the batch size used in each iteration. We also note that the optimal result for an algorithm  can be achieved by a reasonable choosing of $|S_1| = \min \{n,  \epsilon^{-a}\}$, then the optimal SFO can be achieved as the minimum SFO between Finite-sum SFO and Online SFO. We refer readers to \cite{Lei2017,Li2018} for further exploration in this aspect. It is clear in \Cref{smooth_comparison} that the proposed SPIDER$^\textbf{+}$ achieves the best result among all algorithms in term of SFO in both finite-sum and online setting for smooth nonconvex optimization while still maintains a reasonable large step size $O(L^{-1})$, which is comparable to the step size used in GD.
%  
% %%
%Furthermore, with such a delicate algorithm in hand, we further extend it to nonsmooth nonconvex optimization and obtain an significant result. We consider a general constrained nonsmooth nonconvex finite-sum problem
% \begin{align*}
%  \min_{x\in \mathcal{X}} 	\Psi(x)  \defeq  f(x)  + h(x),  \quad f(x) \defeq \frac{1}{n}\sum_{i=1}^{n} f_i(x),  \tag{P2}
% \end{align*}
%where $\mathcal{X}$ is a closed convex set in Euclidean space $\mathbb{R}^d$, $f: \mathcal{X} \rightarrow \mathbb{R} $ is the average of $n$ continuously differentiable functions $f_i: \mathcal{X} \rightarrow \mathbb{R} $, but possibly nonconvex, and $h: \mathcal{X} \rightarrow \mathbb{R} $ is simple convex function, but possibly nonsmooth.  If $h(x) \equiv 0$ and $\mathcal{X} = \mathbb{R}^d$, then this problem reduces to a simple smooth nonconvex problem. However, in many machine learning problems, $h(x)$ is often a nonsmooth  regularizer such that the obtained minimizer $x^\star$ has specific structure. For example, $h(x) = \|x\|_1$  induces sparsity for the obtained minimizer.  We proposed a proximal SPIDER$^\textbf{+}$ algorithm (ProxSPIDER$^\textbf{+}$) and achieves the total gradient complexity of $n^{1/2}\epsilon^{-1}$ to obtain an $\epsilon$-approximate solution, which is the best result in proximal first-order algorithm to the best of our knowledge. We summarize our result in \Cref{comparison_nonsmooth}. For nonsmooth nonconvex optimization, we introduction another oracle the proximal oracle (PO), which is defined as given a point $x$ and the gradient estimator $v$, PO returns the solution of the proximal projection. As shown in \Cref{comparison_nonsmooth} our result improves the previous result by an order of $O(n^{1/6})$ in terms of SFO on finite-sum setting.
%
%
%Furthermore,  we also consider SPIDER$^\textbf{+}$ and ProxSPIDER$^\textbf{+}$ under \emph{online optimization} setting, where the sample size $n$ is too large or even infinite. Then, taking a full batch samples at each outer loop is not efficient or even impossible. In fact, to obtain an $\epsilon$ accuracy, the full batch is not necessary. By taking sample size of the outer loop  in the order of $O(\epsilon^{-1/2})$, we show that the total gradient complexity is $O(\epsilon^{-3/2})$ for both \emph{smooth} (P1) and \emph{nonsmooth} (P2) problems to achieve the $\epsilon$ accuracy. Especially, to the best of our knowledge, our result  $O(\epsilon^{-3/2})$ on nonsmooth problem is new in literature,  and is the best result in proximal first-order method, which improves the SFO in the previous study in an order of $\epsilon^{1/6}$ on online setting.
%----------------------------------------------------------------------------------------------


 

